Don't Forget Your ABC's: Evaluating the State-of-the-Art in Chat-Oriented Dialogue Systems

Despite tremendous advancements in dialogue systems, stable evaluation still requires human judgments producing notoriously high-variance metrics due to their inherent subjectivity. Moreover, methods and labels in dialogue evaluation are not fully standardized, especially for open-domain chats, with a lack of work to compare and assess the validity of those approaches. The use of inconsistent evaluation can misinform the performance of a dialogue system, which becomes a major hurdle to enhance it. Thus, a dimensional evaluation of chat-oriented open-domain dialogue systems that reliably measures several aspects of dialogue capabilities is desired. This paper presents a novel human evaluation method to estimate the rates of many dialogue system behaviors. Our method is used to evaluate four state-of-the-art open-domain dialogue systems and compared with existing approaches. The analysis demonstrates that our behavior method is more suitable than alternative Likert-style or comparative approaches for dimensional evaluation of these systems.

==> notes/abc-eval-annotation-subtasks.tex <==
The 8 annotation subtasks are:

\paragraph{Interpretability} Identifies bot utterances that are difficult to understand their intended meaning, from causes like ambiguity, nonsensical phrasing, grammar errors, etc. This does not include utterances that are illogical with regard to the context or the world. 
The annotator marks uninterpretable utterances using a checkbox element.
\newline
Labels: \texttt{uninterpretable}

\paragraph{Sociality} Identifies bot utterances that are insulting, hateful, or excessively vulgar.
The annotator marks antisocial utterances using a checkbox element.
\newline
Labels: \texttt{antisocial}

\paragraph{Empathy} Identifies bot utterances that show an understanding - or lack of understanding - of someone's emotions, including both the user and others referenced in the conversation.
The annotator selects the appropriate case out of three mutually exclusive options using radio buttons: empathetic, unempathetic, or not applicable (for cases where there is no emotional value). Selecting an option is required.
\newline
Labels: \texttt{empathetic, lack of empathy}

\paragraph{Personal Information} Identifies bot utterances that share information about the bot's preference information or elements of their personal life.
The annotator selects the appropriate case(s) out of two options using checkbox elements: preference or life. The options are not mutually exclusive and selecting an option is not required, since it is possible for an utterance to share one type of information, both types, or neither.
\newline
Labels: \texttt{preference info, life info}

\paragraph{Knowledge} Identifies bot utterances that reference factual knowledge about the world, and label whether the referenced knowledge is accurate or inaccurate.
The annotator first decides whether some factual knowledge has been indicated by the bot's utterance through a checkbox element. If the checkbox is marked, then the annotator must discriminate from four cases using radio buttons: accurate fact usage, inaccurate fact usage, misleading statement, or uncertain. If the annotator selects the uncertain option, then they are instructed to spend a minute searching the Internet for sources relevant to the claimed facts. After they perform the search, they are instructed to discriminate between four cases again using radio buttons: accurate  fact usage, inaccurate fact usage, controversial fact (e.g. credible sources both in support and against the fact), and inconclusive.
\newline
Labels: \texttt{fact usage, fact contradiction}

\paragraph{Commonsense} Identifies bot utterances that contradict common knowledge, which is knowledge that can be understand to be generally agreed upon and learned through direct experience rather than being taught explicitly. This includes violations of commonsense, making unfounded assumptions, inconsistencies, and so on.
The annotator marks violations of commonsense using a checkbox element.
\newline
Labels: \texttt{common knowledge contradiction}

\paragraph{Consistency} Identifies bot utterances that are inconsistent, either within utterance or within the dialogue context. 
The annotator selects the appropriate case(s) out of three options using a dropdown selector: self contradiction, partner contradiction, and redundant. Any combination of the three options can be selected for each bot utterance.
\newline
Labels: \texttt{self contradiction, partner contradiction, redundant}

\paragraph{Dialogue Flow}  Categorize bot utterances based on their appropriateness to the dialogue context, covering the facets of relevance, partner acknowledgements, and conversation topics.
The annotator answers three questions using radio buttons for the bot utterance. The first question addresses whether the bot appropriately acknowledges the user's previous utterance including an option for there being no need to directly acknowledge the user (e.g. for cases where there is no meaningful content in the user's previous utterance such as if the user themself provides an acknowledgement like ok, sounds good, etc.). The second question addresses whether the bot is introducing a new topic, introducing a new talking point that is still within the current conversational topic, or following up on the user's previous utterance. The third question posits whether the bot response is relevant to the current discussion or if it is an irrelevant interruption. 
\newline
Labels: \texttt{ignore, irrelevant, follow-up, topic switch}

==> notes/bot-analysis-tables.tex <==
% \begin{table}[htbp]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|l|l|l|l}
% bot & label & mean & CI low & CI high \\ \hline
% rerank\_blender & informative & 3.940 & 3.751 & 4.129 \\ \hline
% rerank\_blender & engaging & 3.870 & 3.662 & 4.078 \\ \hline
% rerank\_blender & proactive & 3.820 & 3.616 & 4.024 \\ \hline
% rerank\_blender & emotional & 3.810 & 3.601 & 4.019 \\ \hline
% rerank\_blender & consistent & 3.670 & 3.432 & 3.908 \\ \hline
% rerank\_blender & relevant & 3.600 & 3.387 & 3.813 \\ \hline
% rerank\_blender & grammatical & 3.470 & 3.251 & 3.689 \\ \hline
% rerank\_blender & quality & 3.230 & 3.031 & 3.429 \\ \hline
% emora & grammatical & 4.020 & 3.871 & 4.169 \\ \hline
% emora & proactive & 3.940 & 3.745 & 4.135 \\ \hline
% emora & consistent & 3.910 & 3.682 & 4.138 \\ \hline
% emora & engaging & 3.750 & 3.573 & 3.927 \\ \hline
% emora & emotional & 3.610 & 3.394 & 3.826 \\ \hline
% emora & informative & 3.520 & 3.357 & 3.683 \\ \hline
% emora & relevant & 3.510 & 3.318 & 3.702 \\ \hline
% emora & quality & 3.420 & 3.268 & 3.572 \\ \hline
% blender2\_3B & emotional & 4.340 & 4.177 & 4.503 \\ \hline
% blender2\_3B & grammatical & 4.210 & 4.040 & 4.380 \\ \hline
% blender2\_3B & relevant & 4.040 & 3.851 & 4.229 \\ \hline
% blender2\_3B & engaging & 3.960 & 3.784 & 4.136 \\ \hline
% blender2\_3B & proactive & 3.840 & 3.651 & 4.029 \\ \hline
% blender2\_3B & informative & 3.680 & 3.489 & 3.871 \\ \hline
% blender2\_3B & quality & 3.590 & 3.401 & 3.779 \\ \hline
% blender2\_3B & consistent & 3.480 & 3.207 & 3.753 \\ \hline
% bart\_fid\_rag\_bcb & informative & 3.830 & 3.645 & 4.015 \\ \hline
% bart\_fid\_rag\_bcb & grammatical & 3.780 & 3.598 & 3.962 \\ \hline
% bart\_fid\_rag\_bcb & relevant & 3.600 & 3.367 & 3.833 \\ \hline
% bart\_fid\_rag\_bcb & emotional & 3.560 & 3.319 & 3.801 \\ \hline
% bart\_fid\_rag\_bcb & engaging & 3.230 & 2.994 & 3.466 \\ \hline
% bart\_fid\_rag\_bcb & consistent & 3.030 & 2.745 & 3.315 \\ \hline
% bart\_fid\_rag\_bcb & quality & 3.000 & 2.813 & 3.187 \\ \hline
% bart\_fid\_rag\_bcb & proactive & 2.880 & 2.656 & 3.104
% \end{tabular}%
% }
% \caption{Average dialogue-level Likert ratings on 8 dimensions from 100 conversations annotated by Surge workforce.}
% \label{tab:bot_likert}
% \end{table}

% \begin{table}[htbp]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|l|l|l|l}
% bot & label & mean & CI low & CI high \\ \hline
% rerank\_blender & emotional & 4.213 & 4.160 & 4.265 \\ \hline
% rerank\_blender & consistent & 4.034 & 3.972 & 4.096 \\ \hline
% rerank\_blender & grammatical & 4.000 & 3.946 & 4.054 \\ \hline
% rerank\_blender & engaging & 3.823 & 3.762 & 3.885 \\ \hline
% rerank\_blender & relevant & 3.741 & 3.675 & 3.806 \\ \hline
% rerank\_blender & informative & 3.728 & 3.673 & 3.783 \\ \hline
% rerank\_blender & proactive & 3.644 & 3.582 & 3.706 \\ \hline
% rerank\_blender & quality & 3.318 & 3.258 & 3.378 \\ \hline
% emora & grammatical & 4.533 & 4.499 & 4.567 \\ \hline
% emora & consistent & 4.140 & 4.081 & 4.199 \\ \hline
% emora & emotional & 3.973 & 3.918 & 4.028 \\ \hline
% emora & engaging & 3.879 & 3.823 & 3.936 \\ \hline
% emora & relevant & 3.797 & 3.731 & 3.863 \\ \hline
% emora & proactive & 3.760 & 3.702 & 3.819 \\ \hline
% emora & quality & 3.521 & 3.459 & 3.583 \\ \hline
% emora & informative & 3.194 & 3.133 & 3.254 \\ \hline
% blender2\_3B & grammatical & 4.646 & 4.610 & 4.683 \\ \hline
% blender2\_3B & emotional & 4.220 & 4.169 & 4.270 \\ \hline
% blender2\_3B & relevant & 4.190 & 4.130 & 4.249 \\ \hline
% blender2\_3B & consistent & 4.089 & 4.026 & 4.151 \\ \hline
% blender2\_3B & engaging & 3.958 & 3.901 & 4.015 \\ \hline
% blender2\_3B & quality & 3.808 & 3.748 & 3.868 \\ \hline
% blender2\_3B & proactive & 3.575 & 3.519 & 3.632 \\ \hline
% blender2\_3B & informative & 3.440 & 3.389 & 3.492 \\ \hline
% bart\_fid\_rag\_bcb & grammatical & 4.311 & 4.263 & 4.358 \\ \hline
% bart\_fid\_rag\_bcb & emotional & 4.024 & 3.963 & 4.084 \\ \hline
% bart\_fid\_rag\_bcb & consistent & 3.936 & 3.867 & 4.005 \\ \hline
% bart\_fid\_rag\_bcb & relevant & 3.896 & 3.827 & 3.964 \\ \hline
% bart\_fid\_rag\_bcb & informative & 3.796 & 3.742 & 3.849 \\ \hline
% bart\_fid\_rag\_bcb & engaging & 3.621 & 3.553 & 3.689 \\ \hline
% bart\_fid\_rag\_bcb & quality & 3.343 & 3.277 & 3.410 \\ \hline
% bart\_fid\_rag\_bcb & proactive & 2.946 & 2.886 & 3.006
% \end{tabular}%
% }
% \caption{Average turn-level Likert ratings on 8 dimensions from 100 conversations annotated by Surge workforce.}
% \label{tab:bot_likert_turn}
% \end{table}

% \begin{table}[htbp]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|l|l|l|l}
% bot & label & proportion & CI low & CI high \\ \hline
% rerank\_blender & empathetic & 0.435 & 0.410 & 0.460 \\ \hline
% rerank\_blender & follow up & 0.419 & 0.395 & 0.444 \\ \hline
% rerank\_blender & preference info & 0.309 & 0.286 & 0.333 \\ \hline
% rerank\_blender & topic switch & 0.253 & 0.231 & 0.275 \\ \hline
% rerank\_blender & life info & 0.248 & 0.227 & 0.270 \\ \hline
% rerank\_blender & correct fact & 0.218 & 0.198 & 0.240 \\ \hline
% rerank\_blender & commonsense contradiction & 0.189 & 0.170 & 0.210 \\ \hline
% rerank\_blender & irrelevant & 0.177 & 0.158 & 0.197 \\ \hline
% rerank\_blender & incorrect fact & 0.176 & 0.158 & 0.196 \\ \hline
% rerank\_blender & lack of empathy & 0.085 & 0.072 & 0.100 \\ \hline
% rerank\_blender & ignore & 0.079 & 0.067 & 0.094 \\ \hline
% rerank\_blender & partner contradiction & 0.062 & 0.051 & 0.075 \\ \hline
% rerank\_blender & self contradiction & 0.043 & 0.034 & 0.055 \\ \hline
% rerank\_blender & redundant & 0.037 & 0.029 & 0.048 \\ \hline
% rerank\_blender & uninterpretable & 0.021 & 0.015 & 0.030 \\ \hline
% rerank\_blender & antisocial & 0.007 & 0.004 & 0.012 \\ \hline
% emora & empathetic & 0.413 & 0.389 & 0.438 \\ \hline
% emora & follow up & 0.404 & 0.380 & 0.429 \\ \hline
% emora & topic switch & 0.290 & 0.268 & 0.314 \\ \hline
% emora & preference info & 0.246 & 0.225 & 0.268 \\ \hline
% emora & life info & 0.204 & 0.184 & 0.225 \\ \hline
% emora & irrelevant & 0.148 & 0.131 & 0.167 \\ \hline
% emora & lack of empathy & 0.143 & 0.126 & 0.161 \\ \hline
% emora & commonsense contradiction & 0.118 & 0.103 & 0.135 \\ \hline
% emora & ignore & 0.117 & 0.102 & 0.134 \\ \hline
% emora & correct fact & 0.104 & 0.089 & 0.120 \\ \hline
% emora & partner contradiction & 0.062 & 0.051 & 0.076 \\ \hline
% emora & redundant & 0.056 & 0.045 & 0.069 \\ \hline
% emora & self contradiction & 0.007 & 0.004 & 0.013 \\ \hline
% emora & incorrect fact & 0.001 & 0.000 & 0.005 \\ \hline
% emora & antisocial & 0.001 & 0.000 & 0.004 \\ \hline
% emora & uninterpretable & 0.001 & 0.000 & 0.004 \\ \hline
% blender2\_3B & follow up & 0.621 & 0.597 & 0.645 \\ \hline
% blender2\_3B & empathetic & 0.425 & 0.401 & 0.450 \\ \hline
% blender2\_3B & preference info & 0.382 & 0.358 & 0.407 \\ \hline
% blender2\_3B & life info & 0.260 & 0.239 & 0.283 \\ \hline
% blender2\_3B & correct fact & 0.217 & 0.197 & 0.238 \\ \hline
% blender2\_3B & commonsense contradiction & 0.162 & 0.144 & 0.181 \\ \hline
% blender2\_3B & topic switch & 0.157 & 0.140 & 0.177 \\ \hline
% blender2\_3B & irrelevant & 0.100 & 0.086 & 0.117 \\ \hline
% blender2\_3B & ignore & 0.089 & 0.075 & 0.104 \\ \hline
% blender2\_3B & redundant & 0.076 & 0.064 & 0.091 \\ \hline
% blender2\_3B & self contradiction & 0.068 & 0.056 & 0.081 \\ \hline
% blender2\_3B & partner contradiction & 0.067 & 0.055 & 0.081 \\ \hline
% blender2\_3B & lack of empathy & 0.056 & 0.045 & 0.068 \\ \hline
% blender2\_3B & incorrect fact & 0.009 & 0.005 & 0.015 \\ \hline
% blender2\_3B & antisocial & 0.004 & 0.002 & 0.009 \\ \hline
% blender2\_3B & uninterpretable & 0.001 & 0.000 & 0.005 \\ \hline
% bart\_fid\_rag\_bcb & follow up & 0.634 & 0.609 & 0.658 \\ \hline
% bart\_fid\_rag\_bcb & preference info & 0.394 & 0.369 & 0.418 \\ \hline
% bart\_fid\_rag\_bcb & correct fact & 0.356 & 0.332 & 0.380 \\ \hline
% bart\_fid\_rag\_bcb & empathetic & 0.333 & 0.309 & 0.357 \\ \hline
% bart\_fid\_rag\_bcb & life info & 0.267 & 0.245 & 0.289 \\ \hline
% bart\_fid\_rag\_bcb & commonsense contradiction & 0.217 & 0.197 & 0.238 \\ \hline
% bart\_fid\_rag\_bcb & incorrect fact & 0.147 & 0.131 & 0.166 \\ \hline
% bart\_fid\_rag\_bcb & lack of empathy & 0.146 & 0.129 & 0.164 \\ \hline
% bart\_fid\_rag\_bcb & self contradiction & 0.117 & 0.102 & 0.134 \\ \hline
% bart\_fid\_rag\_bcb & topic switch & 0.115 & 0.100 & 0.132 \\ \hline
% bart\_fid\_rag\_bcb & ignore & 0.114 & 0.099 & 0.131 \\ \hline
% bart\_fid\_rag\_bcb & irrelevant & 0.110 & 0.095 & 0.127 \\ \hline
% bart\_fid\_rag\_bcb & partner contradiction & 0.071 & 0.059 & 0.085 \\ \hline
% bart\_fid\_rag\_bcb & redundant & 0.054 & 0.044 & 0.067 \\ \hline
% bart\_fid\_rag\_bcb & uninterpretable & 0.013 & 0.008 & 0.020 \\ \hline
% bart\_fid\_rag\_bcb & antisocial & 0.001 & 0.000 & 0.005
% \end{tabular}%
% }
% \caption{Average proportion of behavior labels from 100 conversations annotated by Surge workforce.}
% \label{tab:bot_behavior_rates}
% \end{table}

==> notes/dimensions_table.tex <==
\begin{table}[htbp!]
\centering
  \begin{small}
  \begin{tabular}{ p{0.25\columnwidth} | l | p{0.52\columnwidth} }
  \hline
  \bf Dimension & \bf Tag & \bf Definition \\
  \hline
  Grammaticality & \tt Gra & Responses are free of grammatical and semantic errors \\
  \hline
  Relevance & \tt Rel & Responses are on-topic with the immediate dialogue history \\
  \hline
  Informativeness & \tt Inf & Responses produce unique and non-generic information that is specific to the dialogue context \\
  \hline
  Emotional Understanding & \tt Emo & Responses indicate an understanding of the user's current emotional state and provide an appropriate emotional reaction based on the current dialogue context  \\
  \hline
  Engagingness & \tt Eng & Responses are engaging to user and fulfill the particular conversational goals implied by the user \\
  \hline
  Consistency & \tt Con & Responses do not produce information that contradicts other information known about the system \\
  \hline
  Proactivity & \tt Pro & Responses actively and appropriately move the conversation along different topics \\
  \hline
  Quality & \tt Qua & The overall quality of and satisfaction with the dialogue \\
  \hline
  \end{tabular}
  \end{small}
  
  \caption{Descriptions and shorthand symbols of the 8 human evaluation dimensions, adapted from \cite{Finch:20}.}
  \label{tab:dims}
\end{table}

==> notes/evaluation-analysis-2.tex <==
Interestingly, the results of the evaluations do not seem to agree with one another when comparing relative bot performances. Although Dialogue Likert and Turn Likert suggest that Blender2 ranks above the rest, with the highest overall quality ratings and the highest rating on several of the other evaluation dimensions, this ranking is not supported by the Comparative results. Instead, Emora and Blender+Decode seem to be vying for the top position in the Comparative evaluation. It is interesting to see that even though the same evaluation dimensions are used for these three evaluation methodologies, they do not result in the same final assessments of the bots.

Indeed, there seems to be a large discrepancy between the Likert-based evaluations and the Comparative evaluation. Although the relative bot rankings between the Dialogue Likert and Turn Likert evaluations are quite similar, with differences arising between bots that are not much different along a certain dimension, the same cannot be said between Likert and Comparative evaluations. Comparative evaluation suggests a different relative ordering of the bots for each dimension, with smaller magnitudes of differences between the bots. For example, the Overall Quality and Relevance of each bot in the Comparative setup is quite similar to one another, in contrast to the results in Dialogue Likert and Turn Likert which overwhelming are in favor of Blender2. These results call into question the synergy between Comparative and Dialogue Likert evaluations, since it seems that they do not produce the same results as one another. In addition, these results do not present convincing evidence that Comparative is a more effective evaluation strategy, as it actually seems less capable of detecting differences between bots compared to Dialogue Likert for the bots in this study. This is in great contrast to previous works (Acute eval, beyond likert dialogue rating) that claim to overcome the disadvantages of Likert evaluation using a Comparative setup, suggesting that there remains work to be done to truly understand the limitations and benefits of each evaluation.

With this incongruency in mind, we elect to look to the results of ABC-Eval to understand the strengths and weaknesses of the evaluated bots, especially as it also provides a higher degree of granularity and interpretability of specific bot behaviors.

==> notes/evaluation-analysis.tex <==
\section{Evaluation Metric Assessment}

\subsection{Power Analysis}

For each label type, show the effect size (cohens d) and statistical power (post-hoc beta) we got for every pair of compared bots. For example, an entry "behavior consistency, blender2 vs emora: 1.0, 70\%" means blender2's consistency sample statistic was one standard deviation higher than emora's (on the distribution of sample statistics), and 70\% of 100-conversation-per-bot samples will reveal a statistically significant difference in the consistency proportion between blender2 and emora with a p value of $<=$0.05. Takeaway: evaluation label X is good/bad/better/worse at detecting differences between bots than evaluation label Y.

\subsection{Predictive Validity}

For each label, show predictiveness (coefficient and $r^2$) of label to predict the quality (interactive likert dialogue score, static likert dialogue score, average likert turn quality, interactive quality comparison, static quality comparison) of a particular dialogue. Takeaway: label X is/is not important with respect to the quality of the dialogue.

For each label, show relative importance (coefficient) of the label to predict quality in a stepwise linear regression model containing all labels, just behavior labels, just likert turn labels, just likert dialogue labels. Takeaway: label X is does/does not give additional information about the dialogue quality above and beyond the other labels.

\subsection{Inter-label Correlations}

Label correlation matrix. Takeaway: Labels X and Y should relate (e.g. behavioral consistency and likert consistency), but they do/do not. 

(Is this correlation matrix important?)


\subsection{Annotation Error Analysis}

Sample 100+ disagreements to do analysis.

For each explanation for disagreement (e.g. nonsensical bot response caused annotator to mark "antisocial"), show \% of annotation disagreements in that category (pie chart?).

==> notes/literature_survey_log.tex <==
\section{Chatbot Error Analysis}

Searches:
\begin{enumerate}
    \item Who cited Higashinaka paper
    \item chatbot error analysis
    \item 
\end{enumerate}

==> notes/model-selection.tex <==
Our goals for dialogue model selection are two-fold. First, our goal is to select models that are state of the art in conversation modelling. Second, we want to ensure variety in the dialogue approaches of the models in order to better validate the evaluation methods (TODO - something about robustness).

We identify 4 focal directions of dialogue work in the recent literature that we use as categories from which we select dialogue models. For each of the 4 categories, we conducted a literature review with the goal of identifying candidate dialogue models to use in our study. The criteria we used to make our selection for this first selection stage is as follows:

\begin{enumerate}
    \item The model must convincingly demonstrate state-of-the-art performance in a task related to the theme.
    \item The model implementation must be provided with either a trained English version available or straightforward procedure to replicate the trained model for English
    \item The response latency must be less than 5 seconds, on average, on modern GPU hardware.
\end{enumerate}

% \subsection{Bot Pilot}

% To include in Section 4 "Model Selection"

% Quality (average likert score, proportion compared favorably to other bots) per bot in the conversation collection pilots. (table with subdivisions to show model focus, e.g. empathetic chat, consistency, info)

% Bots include Blender2, DECODE-reranked blender2, DECODE-reranked blender1, Emora, Bart-FiD-RAG, CEM, DukeNet

% Takeaways: 

% 1. response generation is not the same task as interactive chat, as response generation models like CEM struggle to hold a real conversation (example conversation?)

% 2. Blender2, DECODE-reranked blender1, Emora, and Bart-FiD-RAG perform the best


\subsection{General Purpose}

There are a few recent models presented that use a large-scale language modelling approach on dialogue-like data, such as Reddit, to train chatbots. These works focus specifically on producing dialogue models that are capable of participating in multi-turn back-and-forth conversations, without necessarily focusing on a specific characteristic of conversation capability. In addition, there has been a large effort to producing an engaging open-domain chatbot system in recent years through competitions including the Amazon Alexa Prize Socialbot Grand Challenge, where most systems tend towards state-machine-based approaches instead.

\paragraph{Candidates} Large-scale language model approaches that fit into this category include DialoGPT (cite), Meena (cite), and Blender/Blender2 (cite). Blender2 outperformed Blender. Blender outperformed Meena. Meena outperformed DialoGPT. Thus, we choose the best-performing Blender2 (2.7 billion parameters) as a candidate in the General Purpose category. On the other side of this category, we also include the best-performing system from the Amazon Alexa Prize Socialbot Grand Challenge (cite). We base this selection on the average user rating in the Final round of judging over all years of the competition, which results in the Emora chatbot (cite) from the 2019 competition being selected as another candidate, with a final round average score of 3.8.

\paragraph{Implementation} An interactive chatting mode for Blender2 is provided through Parlai (cite); however, the internet-search augmented functionality as described in the paper is not provided. Although there is an available alternative internet search server (link/cite) that is compatible with Blender2, it increased the response latency of Blender2 such that it no longer met Criteria 3. As a result, we use the version of Blender2 that does not include the internet search functionality.

We implement a Parlai agent using the interactive chatting mode provided for the Emora system (link).

\subsection{Knowledge-grounded} 

TODO - brief description of knowledge-grounded dialogue models

\paragraph{Candidates} To the best of our knowledge, at the time of selection, ColV (cite) is the state of the art model for knowledge-grounded response generation. However, no model is provided. Thus, we looked to the next best-performing model for our candidate identification within the knowledge-grounded category. DukeNet (cite) and Pipm (cite) each report similar performances on the knowledge-grounded response generation task, which appear to be the next best performances after ColV; however, they do not directly compare to each other. The ColV paper presents results for both DukeNet and Pipm; thus we look to that paper to tiebreak between DukeNet and Pipm. The ColV paper's results suggests that Dukenet may have a performance advantage over Pipm; therefore, we include DukeNet as a candidate model for our study.

Additionally, BART-FiDRAG (cite) was published with compelling performance on knowledge-grounded response generation. However, it did not compare to the previous state of the art models. We included BART-FiDRAG as another candidate for our study in order to make the determination of the state of the art ourselves. 

\paragraph{Implementation} The published code for DukeNet does not provide an interactive chatting mode for interacting with the trained model. As a result, upon careful consideration of the available code and described model architecture, we implemented an interactive chatting mode for trained DukeNet models that maintains the expected knowledge tracking formulation across turns in a dialogue. 

One major limitation of this interactive chatting mode is that the relevant knowledge documents are not predetermined for a given input utterance and context, unlike in the training and evaluation paradigms. In order to remedy this and provide a pool of knowledge documents for DukeNet to use to respond within a dialogue, we use a trained Dense Passage Retrieval model (cite) on the standard 2018 wikipedia dump (cite) as provided through Huggingface to select knowledge at each dialogue turn. Specifically, the DPR model takes as an input query the previous user utterance and outputs the 5 most-relevant documents, which are then split into tokenized sentences using NLTK (cite) and converted into the expected knowledge document format of DukeNet. To the best of our knowledge, this implementation accurately represents the capability of a DukeNet model in an interactive setting. We use the published trained DukeNet model on Wizard of Wikipedia dataset (cite), since this dataset is not restricted to a single topic, unlike the alternative trained DukeNet model on CMU-dog (cite) which is restricted to only the movie topic. We implement a Parlai agent using this trained model and our custom interactive chatting mode.  

On the other hand, for BART-FidRAG, an end-to-end interactive chatting mode is provided through Parlai. We use the default arguments for BART-FidRAG in Parlai, except for the arguments \texttt{compressed-indexer-nprobe} and \texttt{beam-context-block-ngram} which we set to 128 and 3, respectively, following internal testing by the authors to optimize the conversation quality.

% \subsection{Commonsense-grounded}

% TODO - brief description of commonsense-grounded dialogue models

% \paragraph{Candidates} To the best of our knowledge, at the time of selection, MKSE-Dialog (cite) is the state of the art model for commonsense-grounded response generation. However, the provided implementation utilizes a Chinese conversation dataset and there is no clear documentation provided that would have enabled us easily use an English dataset instead. Thus, we exclude this model as it fails to meet Criteria 2. Thus, we looked to the next best-performing model for our candidate identification within the commonsense-grounded category. ConceptFlow (cite) reports the next-best performance after MKSE-Dialog, so we include ConceptFlow as a candidate model for our study.

% It is worth noting that several recent dialogue models that utilize commonsense knowledge are specifically targeting the empathetic response generation task. Because of this, we do not consider them within the commonsense-grounded category; rather, they were considered in our pursuit of candidate identification for the empathy category below. 

% \paragraph{Implementation} The published code for ConceptFlow does not provide an interactive chatting mode for interacting with the trained model. As a result, upon careful consideration of the available code and described model architecture, we implemented an interactive chatting mode for trained ConceptFlow models, which dynamically constructs the expected commonsense data given an input utterance in an ongoing dialogue using the provided data resource files. To the best of our knowledge, this implementation accurately represents the capability of a ConceptFlow model in an interactive setting. Since a trained ConceptFlow model was not provided within the published repository, we also trained our own model to use interactively, using the default arguments from the repository, except for the batch size which we set to 100 for training efficiency. Our final trained model replicated (and surpassed) the recorded results of ConceptFlow in the paper as shown in Table \ref{table:conceptflow_replication}. We implement a Parlai agent using this trained model and our custom interactive chatting mode. 

\subsection{Consistency}

TODO - brief description of consistency-focused dialogue models

\paragraph{Candidates} For the most generalized results, we consider dialogue models that target improving consistency of the system in a general sense, rather than focusing on a specific type of information to enforce consistency on, such as profiles as in PersonaChat (cite) and related work (cite).  To this end, we observe that the work done by (DECODE cite) presents state-of-the-art performance on the general consistency task for dialogue to the best of our knowledge at the time of selection. 

\paragraph{Implementation} Following that paper, we finetune a pretrained classifier and use said classifier to rerank a dialogue model's responses at each turn in the dialogue, such that the least contradictory response is ultimately selected as the final response. 

We follow their best-performing setup to train the classifier, which is to use a pretrained Roberta classifier, which we take from (cite), and finetune it using the structured-utterance approach on the DECODE dataset. We also follow the suggestion from their best-performing results, which is to use a Blender model with a topk inference strategy where k = 40. Although the paper presents results based on Blender, we use Blender2 as it has surpassed the performance of Blender in its original form. 

We implement a custom agent in the Parlai framework which utilizes our finetuned classifier to rerank Blender2 responses within an interactive chatting mode.

\subsection{Empathy}

TODO - brief description of empathy-focused dialogue models

\paragraph{Candidates} As we are interested in end-to-end dialogue models capable of participating in a back-and-forth multi-turn dialogues with users, we focus on dialogue models that produce empathetic responses without requiring an explicit input emotion to be provided when producing a response; rather, these models take an end-to-end response generation approach that may subsume the process of identifying the desired emotion of the response. Within this restriction, the state of the art model for empathetic response generation is CEM (cite) to the best of our knowledge at the time of selection, so we include CEM as a candidate model for our study.

\paragraph{Implementation} The published code for CEM does not provide an interactive chatting mode for interacting with the trained model. As a result, upon careful consideration of the available code and described model architecture, we implemented an interactive chatting mode for trained CEM models. To the best of our knowledge, this implementation accurately represents the capability of a CEM model in an interactive setting. Since a trained CEM model was not provided within the published repository, we also trained our own model to use interactively, using the default arguments from the repository. We implement a Parlai agent using this trained model and our custom interactive chatting mode. 

\subsection{Verification Pilot}

This study is specifically focused on analyzing the current state-of-the-art of dialogue systems. We take the definition of a dialogue system to be any automated model capable of holding mostly sensible long-form multi-turn conversations with human users. This definition of dialogue system does not require models to replicate human conversational capabilities; rather, it assumes a minimum level of competency that must be met. If any model produces responses within a multi-turn conversation that are frequently difficult for most human users to respond to them, such a model does not fit this definition of dialogue system, since they are missing a baseline level of conversational capability. For the purposes of this study, no further analysis is beneficial for dialogue models with such overwhelming and consistent issues, as the overall pattern of their evaluations and labels can be determined from only a few samples. 

Since several of the selected candidate dialogue models did not provide an interactive chatting interface or interactive human evaluation, it was necessary to verify that these selected candidate models can be considered dialogue systems. To this end, we perform a pilot of this study to assess which models pass the dialogue system verification check and will be included in the full implementation of this study.

This pilot follows the setup of Stage 1 of this study, where pairs of conversations are collected along with their Likert and Comparative annotations. All participants are blinded, such that they are unaware of which dialogue model they are conversing with. The pilot participants are students from the author's research lab, including the authors themselves. 

The dialogue models that were included in this pilot were: Blender2, DukeNet, BART-FiDRAG, ConceptFlow, and CEM. Since Blender2+DECODE is a variation of Blender2 that mostly relies on Blender2's response capability, we do not include Blender2+DECODE in the pilot. Using a DECODE-based classifier to rerank the top Blender2 responses should not affect the overall conversation capability of Blender2, so we take the results of Blender2 for Blender2+DECODE as well. We also exclude the Emora system from this pilot, as its competency as a dialogue system was already proved by winning the Alexa Prize 2019.

For the purposes of this pilot, we used the average quality Likert rating received by each model as the verification metric. Any models that received a rating of 2.5 or lower were considered to fail the verification check of their dialogue system suitability, after manual review of their conversations to confirm their low rating was due to glaring and consistent response issues.

The average Likert rating received by each model is shown in Table \ref{tab:bot_pilot_results}. It is clear to see that several models received Likert ratings that indicated their failure as a dialogue system. Specifically, the models CEM, DukeNet, and ConceptFlow failed to pass the verification pilot. As a result, these models are not included in the remainder of this study. The final models for the full study thus become:

\begin{itemize}
    \item Blender2
    \item Emora
    \item BART-FiDRAG
    \item Blender+DECODE
\end{itemize}

\begin{table}[htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\textbf{bot}        & \textbf{mean} & \textbf{CI low} & \textbf{CI high} & \textbf{n} \\ \hline
rerank\_blender     & 3.800         & 3.236           & 4.364            & 10         \\ \hline
emora               & 3.500         & 2.727           & 4.273            & 10         \\ \hline
bart\_fid\_rag\_bcb & 3.400         & 2.709           & 4.091            & 10         \\ \hline
blender2\_3B        & 3.400         & 1.734           & 5.066            & 5          \\ \hline
rerank\_blender2    & 3.300         & 2.343           & 4.257            & 10         \\ \hline
dukenet             & 1.889         & 1.176           & 2.602            & 9          \\ \hline
cem                 & 1.083         & 0.900           & 1.267            & 12        
\end{tabular}%
}
\caption{The bot pilot results for 7 bots, showing the number of collected conversations (n) as well as the average (mean) and 95\% confidence interval (CI low, CI high) of the dialogue-level Likert quality ratings per bot.}
\label{tab:bot_pilot_results}
\end{table}


% \subsection{General Purpose}

% Blender outperformed Meena, which outperformed DialoGPT. GPT-3 is not dialogue-targeted and is not freely available as an interactive model (openai api with monetary cost).

==> notes/sensitivity_table_other_designstex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
% \textbf{Evaluation} & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & behavior & comparative & comparative & comparative & comparative & comparative & comparative & comparative & comparative & likert dialogue & likert dialogue & likert dialogue & likert dialogue & likert dialogue & likert dialogue & likert dialogue & likert dialogue & likert turn & likert turn & likert turn & likert turn & likert turn & likert turn & likert turn & likert turn \\ \hline
\textbf{Label} & $\sim$Soc$_b$ & $\sim$Com$_b$ & Fac$_b$ & Emp$_b$ & Fol$_b$ & Ign$_b$ & $\sim$Fac$_b$ & $\sim$Rel$_b$ & $\sim$Emp$_b$ & Lif$_b$ & $\sim$Par$_b$ & Pre$_b$ & Red$_b$ & $\sim$Sel$_b$ & Top$_b$ & $\sim$Int$_b$ & Con$_c$ & Emo$_c$ & Eng$_c$ & Gra$_c$ & Inf$_c$ & Pro$_c$ & Qua$_c$ & Rel$_c$ & Con$_d$ & Emo$_d$ & Eng$_d$ & Gra$_d$ & Inf$_d$ & Pro$_d$ & Qua$_d$ & Rel$_d$ & Con$_t$ & Emo$_t$ & Eng$_t$ & Gra$_t$ & Inf$_t$ & Pro$_t$ & Qua$_t$ & Rel$_t$ \\ \hline
\textbf{0.001} & 0 & 4 & 5 & 3 & 4 & 1 & 4 & 3 & 5 & 2 & 0 & 5 & 1 & 5 & 4 & 4 & 2 & 0 & 1 & 0 & 2 & 2 & 0 & 0 & 1 & 3 & 2 & 2 & 1 & 3 & 2 & 1 & 1 & 4 & 3 & 6 & 5 & 4 & 5 & 4 \\ \hline
\textbf{0.01} & 0 & 4 & 5 & 3 & 4 & 3 & 5 & 4 & 5 & 3 & 0 & 5 & 1 & 5 & 5 & 4 & 2 & 0 & 1 & 0 & 3 & 3 & 0 & 0 & 2 & 3 & 3 & 3 & 2 & 3 & 3 & 3 & 3 & 4 & 4 & 6 & 5 & 4 & 5 & 4 \\ \hline
\textbf{0.05} & 1 & 4 & 5 & 3 & 4 & 4 & 5 & 5 & 5 & 3 & 0 & 5 & 5 & 6 & 6 & 4 & 4 & 2 & 3 & 0 & 4 & 5 & 0 & 1 & 3 & 3 & 3 & 4 & 3 & 3 & 3 & 3 & 3 & 4 & 5 & 6 & 6 & 5 & 5 & 4 \\ \hline
\end{tabular}%
}
\caption{The number of bot pairs that are significantly different from one another with regard to the evaluation label at three sensitivity levels (0.001, 0.01, 0.05), according to t-test. The maximum value for any entry is 6 as there are 6 bot-pairs in this work.}
\label{tab:sensivity}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> old_latex_files/evaluation_related_works.tex <==
\section{Evaluation Methods}

This section summarizes the existing methods for evaluating chat models, and indicates which methods we chose to include in our study. 

\subsection{Existing Methods}

There is an overall lack of standardization in chat model evaluation, with many distinct methods proposed \cite{finch_towards:20}. Existing evaluation methods can be broadly divided into two groups: (1) single-turn evaluations, where models are given a dialogue context and are judged on their ability to produce an appropriate response \cite{ghandeharioun:19, shuster:21, song:21}; and (2) multi-turn evaluations, which test a model’s ability to interactively produce a sequence of responses to some dialogue partner’s input \cite{ghandeharioun:19, roller:21, komeili:22}. While single-turn evaluation is more cost-effective, we observe that this kind of evaluation is inadequate for estimating a model’s ability to converse interactively (see TAB in SEC) which has also been suggested by \cite{mehri:21}; therefore, we only consider multi-turn evaluation methods in our study.

Dialogue evaluation methods can also be categorized into automatic evaluations that use a formula \cite{papineni:02, banerjee:05} or model \cite{lowe:17, sinha:20, zhang_d-score:21} to measure characteristics of a model’s responses, and human evaluations that incur the cost of manually labeling model responses \cite{finch_towards:20, li_acute-eval:19}. Existing automatic evaluations have been shown to be biased \cite{liu:16} and gameable \cite{deriu:22, sai:19}, and developing automatic metrics for dialogue that agree with human judgements is an active research problem \cite{yeh:21}. Most works therefore include human evaluations when presenting novel chat models \cite{finch_towards:20}. 

Human evaluations can be either interactive, where human interactors also serve as evaluators to judge model performance \cite{roller:21, adiwardana:20, shuster:22}, or static, where human evaluators make judgements on conversations they did not participate in themselves \cite{mehri:21}. Given the wide variety of proposed evaluation approaches and the current challenges facing automatic methods, we narrow the scope of our analyses to human evaluation methods only, and leave it to future work to further investigate and validate automatic methods. Furthermore, we focus especially on static human evaluation methods since they are easier to perform in practice.

Human evaluation methods can ask evaluators to label characteristics of a dialogue as a whole (dialogue-level) \cite{saleh:20, smith:20}, or to label the characteristics of individual turns within a dialogue \cite{ghazarian:22, xu:22}, with the labeling decision itself coming in three popular styles: (1) ratings on likert scales \cite{saleh:20, smith:20} \footnote{\cite{santhanam:19} show that continuous scales are an alternative to ordinal likert scales, although this method is very uncommon in dialogue evaluation}; (2) comparative decisions that ask the evaluator to choose which dialogue or turn is a better match of the label definition \cite{zhou:18, li_acute-eval:19, wu_topicka:20}; and (3) classifications, where evaluators are asked to determine which class a dialogue or turn belongs to from a set of class definitions, such as error categories \cite{higashinaka:21, xu:22}. 

To have confidence that an evaluation measure yields useful information, its replicability and sensitivity require validation. Replicability and interpretability is often estimated via inter-annotator agreement measures; however, there are few works that compare the sensitivity of alternative human evaluation approaches. \cite{li_acute-eval:19} investigate the differences in sensitivity between dialogue-level likert and comparative evaluations for 4 human dimensions across several bots and present cost effectiveness for one human dimension on one bot-pair, although they reuse likert rating results from past works for this comparison which results in sparsity and data incongruence. Although they present a small-scale agreement analysis for their question optimization, they fail to provide IAA for their full study. \cite{smith:22} compare the win rates, variability, and cost effectiveness between combinations of pairwise/likert and single-turn/multi-turn evaluations for 3 human dimensions on 4 variants of Blender, although they fail to present IAA. \cite{deriu:20} propose a human evaluation in which bot comparisons are achieved through pairwise win rates and survival analysis techniques using human judgements of bot-ness of each speaker in variable-length bot-bot conversations. They utilize this evaluation on many bots and present statistically significant results between bot-pairs, annotator agreement, explicit annotation timings, and cost-effectiveness; however, they fail to provide a direct comparison to previous human evaluation methods in these analyses. \cite{lee:20} presents the IAA and statistical significance of their evaluation results across 10 chatbots using the comparative human evaluation platform ChatEval \cite{sedoc:19}; however, they fail to provide a direct comparison to previous human evaluation methods. \cite{sedoc:20} apply Item Response Theory to comparative human bot evaluation across several bots and present IAA, standard error, and statistical significance results; however, they fail to provide a direct comparison to previous human evaluation methods in these analyses. \cite{ji:22} present modifications to traditional likert scales using a continuous (0-100) rating scale, score standardization, and an annotator quality check. They perform a replicability study and present explicit collection timings, IAA, and statistical significance testing of 4 bots; however, they fail to provide a direct comparison to previous human evaluation methods. \cite{zhang_human-machine:21} propose a hybrid human-machine evaluation paradigm in which evaluation decisions are assigned to either a human or an automated system depending on estimated machine certainty and human effort. They evaluate on a response classification task only and, as such, it is unclear the applicability of such an evaluation strategy to the task of chatbot evaluation. 

Furthermore, although it is widely accepted that evaluations of several characteristics of chat is preferred over an evaluation of overall quality alone, few works attempt an analysis of the relevant characteristics that should be used in a high-coverage set of evaluation labels. \cite{see:19} perform an analysis of the importance of repetition, specificity, relevance, and interrogativeness by directly manipulating these characteristics as parameters of their chatbot implementation, but they find small differences (if any) between the various aspects. \cite{finch_towards:20} similarly construct a set of commonly-used likert-style labels via literature review and show the relationship between those labels and overall quality for 100 Alexa Prize conversations from the Emora bot without any significance testing. \cite{venkatesh:18} show a correlation analysis between 2 human-annotated metrics of engagement and coherence to the human quality rating for a large set of conversations across several bots from the Alexa Prize. Both \cite{higashinaka:21} and \cite{sanguinetti:20} construct taxonomies of errors for chatbots and customer-service bots, respectively, with reported IAA, but do not validate the coverage or sensitivity of the final label set. \cite{deriu:20} report the influence of human-annotated fluency, specify, and sensibleness on bot survival.  \cite{ji:22} present the correlation between several dialogue characteristics (interestingness, funness, consistency, fluency, roboticness, repetitiveness, on-topic-ness) and overall quality.

Some approaches to automated metric development include correlational analyses of collected human annotations on dialogue characteristics to overall dialogue quality. \cite{mehri_unsupervised:20} propose a wide range of turn- and dialogue-level characteristics which are annotated by human evaluators on 124 conversations from humans, Meena, and Mtsuku \footnote{\href{https://venturebeat.com/mobile/mitsuku-chatbot-wins-most-humanlike-a-i-loebner-prize-again/}{https://venturebeat.com/mobile/mitsuku-chatbot-wins-most-humanlike-a-i-loebner-prize-again/}}. They present IAA, but fail to conduct additional analyses on this evaluation paradigm, notably failing to indicate statistical significance of differences between the 3 speakers. They also present the coefficients of both turn-level and dialogue-level regression models fitted to overall quality for each characteristic. \cite{see:21} identify 7 types of bot errors from an error-analysis of their GPT-2-based generative model of the ChirpyCardinal bot and present regression coefficients for the mistakes from models fitted on identifying next-utterance dissatisfaction types. They present IAA of the errors, but do not present any sensitivity or validation of their error taxonomy, instead acknowledging the lack of coverage from such an error taxonomy due to the reliance on one non-SOTA generative model. \cite{phy:20} collected binary human annotations of understandability, sensibility, and specificity of response generation outputs and report IAA as well as regression coefficients of the characteristics with respect to overall quality, specific to each annotator. \cite{mehri_usr:20} collect human judgements (binary and likert) for understandability, naturalness, context coherence, interestingness, and knowledge incorporation on response generation outputs and report IAA as well as regression coefficients of the characteristics with respect to overall quality, specific to each annotator. They present weak coverage evidence by fitting a regression model to produce the overall score using the characteristics which achieves high correlation between estimated score and true score.

In an effort to construct higher quality datasets for training and evaluation of bots, some works purport the importance of specific dialogue skills to justify their dataset decisions \cite{smith:20, shuster:20}; however, these works do not provide any empirical evidence of the coverage or importance of such proposed skills, rather drawing on general themes from the conversational AI field as a whole.

Based on the review of existing methods we summarize above, we notice that there is an overall lack of comparison and validation across different methods, especially between different styles of human evaluation. Our study addresses this gap by comparing likert-, comparative-, and classification-style human evaluation methods on a wide range of chat characteristics with a detailed look into the coverage of the respective label sets.


\subsection{Selected Methods}
\label{sec:selected_evals}

Given the wide variety of human evaluation methods for chat and lack of analysis on which methods are most valid, we select four static human evaluation methods from previous work for our study: 

\paragraph{Dialogue Likert ($\{tag\}_d$)} 
\label{sec:dialogue-likert}
Annotators provide dialogue-level ratings on a 1 (least) - 5 (most) Likert scale for each of 8 characteristics (Table \ref{tab:dims}) from \cite{finch_towards:20}. We chose this label set since it was produced via a detailed survey of characteristics used in chat evaluation and, in theory, has better coverage than alternatives like the set used in ACUTE-Eval \cite{li_acute-eval:19}. Bot-level metrics are calculated as the mean rating across all bot dialogues.

\paragraph{Turn Likert ($\{tag\}_t$)}
Annotators provide turn-level ratings on a the same Likert scale and characteristics as \sref{sec:dialogue-likert}. Dialogue-level metrics are calculated as the mean rating across all turns for the dialogue. Bot-level metrics are calculated as mean rating across all turns for all bot dialogues.

\paragraph{Comparative ($\{tag\}_c$)}
Annotators select the dialogue in which Speaker 2 better fit a characteristic definition from a side-by-side pair of dialogues for the same characteristics as \sref{sec:dialogue-likert}. A “neither” option to be used only in cases where the evaluator could not distinguish which dialogue was a better fit. Bot-level metrics are calculated both pairwise as win/tie/loss proportions between paired dialogues of specific bot-pairs and on aggregate as win/tie/loss proportions between all pairs of dialogues involving the bot.

\paragraph{Behavior Classification: ABC-Eval ($\{tag\}_b$)}
A novel methodology created by synthesizing the chat characteristics proposed by several previous works into a set of binary, turn-level behavior labels and iteratively refining the evaluation procedure (Table \ref{tab:behavior_labels}). Dialogue-level metrics are calculated as proportion of turns that display the characteristic for the dialogue. Bot-level ratings are calculated as the proportions of turns that display the characteristic over a set of dialogues. We discuss this evaluation approach and its development in detail in the next section (\sref{sec:abc-eval}). 

\begin{table}[htbp!]
\centering
  \begin{small}
  \begin{tabular}{ l | l }

  \bf Dimension & \bf Tag \\
  \hline \hline
  Grammaticality & \tt Gra \\
  \hline
  Relevance & \tt Rel \\
  \hline
  Informativeness & \tt Inf \\
  \hline
  Emotional Understanding & \tt Emo  \\
  \hline
  Engagingness & \tt Eng \\
  \hline
  Consistency & \tt Con \\
  \hline
  Proactivity & \tt Pro \\
  \hline
  Quality & \tt Qua \\

  \end{tabular}
  \end{small}
  
  \caption{Shorthand tags of the 8 characteristics used for likert-style and comparative-style evaluations.}
  \label{tab:dims}
\end{table}


==> old_latex_files/old_sections/0_abstract.tex <==
\begin{abstract}

Chat-oriented dialogue evaluation is notoriously challenging due to the inherent subjectivity in defining the quality of a human-computer chat.
Evaluations that employ human judges to rate conversation quality have become a de-facto standard in this area; however, current human evaluation methodologies are largely unstandardized and often produce unreliable evaluation metrics due to high variance in human judgements. 
In addition, existing evaluation methodologies fail to illuminate the prevalence of undesirable behaviors that are made by current dialogue systems, rendering it difficult to clearly understand the outstanding challenges.
In this work, we propose a novel human evaluation method - ABC-Eval - that seeks to remedy this limitation by having annotators judge chatbot responses on important defined behaviors, such as self-contradiction, topic switching, and more.
Moreover, we present a study that compares the existing human evaluation methods as well as ABC-Eval by applying these various methodologies to four diverse chat models that have achieved state-of-the art performance in a relevant chat-oriented dialogue task.
The results of our study show the merits and limitations of each evaluation methodology, by exploring the reliability, sensitivity, and cost of each method we investigate, and also serve to reveal the most pressing issues present in current chatbot models.
Using the findings we present, future work in chat-oriented dialogue modelling will be better informed in both (1) the current limitations of current chatbot models and their relative importance, and (2) choosing a suitable evaluation methodology for their research goals.

\end{abstract}

==> old_latex_files/old_sections/abc-eval.tex <==
\section{ABC-Eval}
\label{sec:behavior-evaluation}

We present ABC-Eval: (A)nnotation of (B)ehaviors in (C)onversation Evaluation, a chatbot evaluation procedure that measures the rate at which the chatbot expresses certain behaviors such as contradicting itself, sharing its preferences, or ignoring the user.
This is accomplished through the human annotation of a set of conversations collected between the chatbot-under-evaluation and a random sample of users.

\subsection{Evaluation Procedure}

\input{tex/fig/behavior-labels}

ABC-Eval is composed of 8 independent annotation subtasks, each with its own training and screening session. Annotators elect to complete one subtask at a time and are given a random dialogue to be annotated. In total, there are 16 binary behavior labels as shown in Table \ref{tab:behavior_labels}, but each subtask involves annotating a conversation for only a small number (1-4) of closely related behavior labels. 

Before annotating any conversation within a specific subtask, we require each annotator to complete that subtask's training. For each subtask, we created three example conversations with gold labels. The example conversations consisted of roughly 30 turns of dialogue between the authors and Blender, that were then heavily hand-modified to improve their suitability as training examples for the subtask. Primarily, bot responses were changed to ensure that the conversation included sufficient subtask-relevant examples of each behavior label included in the subtask, as well as negative cases. Gold labels were assigned to each bot response in each example conversation by the authors. In addition, the authors wrote a short 1-3 sentence explanation each chatbot response to describe why the given gold label is correct.

Annotators complete a training session for a subtask by annotating each of the three example conversations. After each example conversation, the gold labels for the conversation are revealed to the annotator, along with the annotation explanation for each incorrectly labelled chatbot response. The third example conversation acted as a screening task: an annotator must meet a correctness threshold of 2 mistakes or less in order to be eligible as an evaluator for real conversations. 

\subsection{ABC-Eval Development}

\begin{table}[htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|c}
\textbf{} & \textbf{Dialogues} & \textbf{Annotators} & \textbf{Type} & \textbf{$\alpha$} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Pilot 1}} & 4 (full) & 11 (2-3/dia) & Lab (ALL) & 0.18 \\ \cline{2-5} 
\multicolumn{1}{c|}{} & 2 (full) & 4 (2/dia) & Lab (G) & 0.39 \\ \hline
\multirow{2}{*}{Pilot 2} & 6 (subset) & 5 & Lab (ALL) & 0.49 \\ \cline{2-5} 
 & 6 (subset) & 4 & Lab (G) & 0.50 \\ \hline
\multirow{2}{*}{Pilot 3} & 6 (subset) & 4 & Lab (U) & 0.43 \\ \cline{2-5} 
 & 6 (subset) & 4 & Lab (U) & 0.45 \\ 
% Pilot 4 & 20 & 17 & 2 annotators per dialogue; label subset per dialogue & Undergrad & 0.30 \\ \hline  
% Pilot 5 & 8 & 18 & 2 annotators per dialogue; label subset per dialogue & Third-Party & 0.36 \\ \hline   
\end{tabular}%
}
\caption{The distribution of dialogues and annotators for each annotation pilot. Pilot 1 included full label annotation of each dialogue where dialogues were distributed among groups of annotators. Pilots 2 and 3 had a subset of labels annotated for each dialogue, but all annotators annotated each dialogue.  \texttt{$\alpha$}: Krippendorf's alpha, \texttt{U}: Undergraduate annotators, \texttt{G}: Graduate level annotators, \texttt{ALL}: Undergraduate and graduate annotators.}
\label{tab:pilot_stats}
\end{table}

The final design of ABC-Eval arose from a series of piloting rounds of the behavior labels, annotation instructions, and software application used for annotation. Details on each piloting round are provided in Table \ref{tab:pilot_stats}. It is important to note that each annotator performed all of the annotation tasks in one sitting in sequence for each pilot. These piloting rounds are not necessarily directly comparable to one another when taken as a whole, since the annotator groups and dialogues to be annotated varied between each round. Instead, we will discuss below the major takeaways afforded by different splits of the pilots that informed the final design of ABC-Eval. 

\paragraph{Subtask Formulation} 
The decision to format ABC-Eval into several small annotation subtasks, each with a tailored subset of the behavior labels, was made from the results of Pilot 1. In Pilot 1, we divided the initial set of annotation labels into 3 annotation subtasks each with 4-9 labels: errors, information usages (commonsense, world knowledge, etc.), and utterance types (request, presentation, etc.). Each annotator performed the annotation tasks in one sitting in sequence. The overall interannotator agreement was quite low ($\alpha=0.18$), which was concerning. Based on ad-hoc feedback from the pilot annotators, the consensus was that each subtask was overwhelming in the amount of information they were required to keep in their minds at one time. 

For Pilot 2, we increased the number of annotation tasks such that each covered a small and related scope of behavior labels, with 1-4 labels per task. Table \ref{tab:pilot_stats} shows the boost to interannotator agreement between Pilots 1 and 2. However, this agreement increase could have resulted from an increase in the quality of the annotators (as Pilot 2 was composed primarily of annotators with a graduate-level education whereas Pilot 1 was more evenly split between annotators with an undergraduate-level education and graduate-level education). To remove this confound, we calculated the agreement in Pilots 1 and 2 when only considering graduate-level annotators. Although it was less dramatic, there remained an increase in agreement from 0.39 to 0.50, which encouraged the decision to maintain the smaller annotation subtasks. Dividing the annotation into tailored subtasks seemed to reduce the cognitive load on annotators, thus allowing them to perform more accurate annotations per task.

\paragraph{Training and Screening}
Manual analysis of the pilot annotations from Pilots 1 and 2 revealed some recurring annotation mistakes, arising from misunderstandings of the guidelines for the tasks. In an attempt to correct such misunderstandings, a training procedure was introduced for each task, where each annotator was taken through 3 rounds of training and feedback on the task and the final round functioned as a screening mechanism based on the annotation accuracy. To evaluate the utility of this training process, a third pilot was conducted using 4 undergraduates. We observed a general upwards trend in annotation performance between the training rounds for the annotators, suggesting that the training was aiding in the annotation accuracy for the annotators. The final agreements were 0.43 and 0.45 between all annotators and annotators who passed the training, respectively, on the annotated conversations. 

Due to the small nature of this pilot, we are unable to conclude whether this difference is meaningful. However, ad-hoc feedback from the annotators suggested that the training rounds were useful towards their understanding of the tasks, although the amount of training was overwhelming since they had to complete all of the training for all tasks before then moving on to perform the annotation tasks for the real conversations. Accordingly, the decision was made to treat each subtask independently, rather than require all subtasks to be completed for one dialogue in a single sitting for each annotator.

\paragraph{General Revisions}
Throughout each of these pilot rounds as well as some preliminary test runs on the various annotation workforces (\sref{sec:workforces}), the annotation instructions, examples, and training rounds were updated based on manual review of the annotations in an attempt to correct any unclear or misleading information.






==> old_latex_files/old_sections/bot-evaluations.tex <==
\section{Bot Evaluation Results}
\label{sec:bot_evaluation_results}

% Turn length analysis?

% Using Surger data only (for simplicity).

% For each bot, show label metrics for each label (proportion compared favorably, average likert turn score, average likert dialogue score, proportion of turns demonstrating behavior) (column chart). Takeaways: Bot X is better than bot Y at Z.

% Show some case study conversation snippets demonstrating problematic behaviors identified in the literature and their corresponding labelings (e.g. an inconsistent dialogue marked with its consistency likert and behavior labels). Takeaway (visualization of other results): behavior labels reliably target issues identified in recent literature, whereas existing human judgement metrics like likert scores are not as reliable.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{tex/fig/comparative.png}
    \caption{The win-tie-lose proportions of each chatbot against all of the others}
    \label{fig:comparative}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{tex/fig/dialogue_likert.png}
    \caption{Average dialogue-level Likert ratings}
    \label{fig:dialogue_likert}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{tex/fig/turn_likert.png}
    \caption{Average turn-level Likert ratings}
    \label{fig:turn_likert}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{tex/fig/desirable_behavior_rates.png}
    \caption{Average proportion of desirable behavior labels}
    \label{fig:desirable_behaviors}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{tex/fig/undesirable_behavior_rates.png}
    \caption{Average proportion of undesirable behavior labels}
    \label{fig:undesirable behaviors}
\end{figure}


% \begin{figure*}[htb]
% \centering
% \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=\textwidth]{tex/fig/dialogue_likert.png}
%     \caption{Average dialogue-level Likert ratings}
%     \label{fig:dialogue_likert}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=\textwidth]{tex/fig/turn_likert.png}
%     \caption{Average turn-level Likert ratings}
%     \label{fig:turn_likert}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=\textwidth]{tex/fig/comparative.png}
%     \caption{The win-tie-lose proportions of each chatbot against all of the others}
%     \label{fig:comparative}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=\textwidth]{tex/fig/desirable_behavior_rates.png}
%     \caption{Average proportion of desirable behavior labels}
%     \label{fig:desirable_behaviors}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.45\textwidth}
%     \includegraphics[width=\textwidth]{tex/fig/undesirable_behavior_rates.png}
%     \caption{Average proportion of undesirable behavior labels}
%     \label{fig:undesirable behaviors}
% \end{subfigure}
% \hfill
        
% \caption{The results for each bot from each evaluation methodology from 400 conversations annotated by Surge workforce. Error bars denote 95\% confidence interval of Likert ratings, behavior rates, and proportion of wins for \ref{fig:dialogue_likert} and \ref{fig:turn_likert}, \ref{fig:desirable_behaviors} and \ref{fig:undesirable behaviors}, and \ref{fig:comparative} respectively.}
% \label{fig:figures}
% \end{figure*}


We look to the results of ABC-Eval to understand the strengths and weaknesses of the evaluated bots, especially as it provides a higher degree of granularity of specific bot behaviors.

\paragraph{Antisociality and Uninterpretability} 
The production of antisocial utterances and uninterpretable utterances was near-zero for these bots. These are two historically high-profile concerns for within the generative dialogue community that do not seem to be a major concern for these bots. For Emora, this can be explained through its handcrafted nature as the human developers had complete control over the final generations. For the remaining bots, the quantity and quality of the training data in these recent years could account for this accomplishment. In particular for antisociality, it could be the case that the training data does not introduce antisocial interactions very often and thus the bots do not learn to produce them. This finding does not necessarily extend to all chatbots, as they vary on their training data and methodology, but it does provide some reassurance that toxic dialogue interactions can be avoided.

\paragraph{Commonsense}
Violations of commonsense are one of the most frequent problems reported across the 4 bots, ranging from 1-2 utterances from every 10 turns exposing a commonsense contradiction on average. BART-FiDRAG has the highest rate of commonsense violations whereas Emora has the least. To the best of our knowledge, this is the first work to quantify the amount of commonsense violations within chatbots and is the first to empirically expose the prevalence of this erroneous behavior. 

\paragraph{Consistency}
Although the rate of partner and self contradictions is relatively lower than other issues like ignoring and commonsense violations, they tend to occur in 1 utterance every 10 to 20 turns on average for most of the bots, which can degrade the user's experience within the conversation. While all of the bots produce approximately the same rate of partner contradictions (around 1 utterance every 20 turns), there is much higher diversity in the rate of self contradictions between the bots. Emora produces the least self-contradictions (near zero) whereas BART-FiDRAG produces the most (around 1 utterance every 10 turns). Notably, Blender+Decode has the second lowest rate of occurrence, which is congruent with its status as an approach to improving chatbot consistency.

\paragraph{Knowledge}
The rates of correct fact usage reveal that BART-FiDRAG is the most factually-oriented bot with between 3-4 utterances every 10 turns incorporating a correct world fact, which is to be expected according to its underlying dialogue approach. However, BART-FiDRAG also expresses one of the highest rates of incorrect fact usages with about 1 utterance every 10 turns revealing an incorrect world fact. Blender+Decode also produces incorrect facts at a similarly high rate, which is much higher than both Blender2 and Emora who produce near-zero utterances with incorrect facts.

\paragraph{Empathy}
BART-FiDRAG appears to be the bot least capable of empathetic response-giving as it has one of the highest rates of unempathetic responses (about 15\% of the time) and the lowest rates of empathetic responses (about 30\% of the time). The remaining bots produce higher rates of empathy (each about 40\% of the time), although Emora also expresses a high rate of unempathetic responses similar to BART-FiDRAG at about 15\% of the time whereas Blender-based bots are unempathetic less than 10\% of the time with Blender2 producing the least unempathetic responses.

It is also worth noting that these results reveal that a large portion of the user utterances in the collected conversations do not assert an emotional experience that has an expected acknowledgement from the bot. For each bot the combined rate of empathetic and unempathetic responses ranges from approximately 45\% - 55\%, which means that the remaining portion is composed of user utterances for which empathy is not applicable (which was the third option of the relevant ABC-Eval annotation scheme).

\paragraph{Personal Information}
All of the bots share information about their life between 20\% to 30\% of the time during a conversation and about their preferences between 20\% to 40\% of the time, with Emora sharing the least amount in both cases. Although this is somewhat surprising on the surface, since Emora was developed with the specific goal to focus on experiential topics like family and work, it is also the case that a large portion of Emora's utterances are questions to the user. Since the relevant behavior labels in ABC-Eval were coded to cover bot presentations only, the prevalence of life and preference discussions is not represented as completely for Emora as compared to the other bots that do not put such a heavy emphasis on question-asking. 

\paragraph{Dialogue Coherence}
Ignoring the user seems to be relatively frequent, occurring about once every 10 utterances across the bots with the Blender-based models ignoring the least often. Comparatively, redundancy is much less of an issue, occurring about once every 20 utterances with Blender2 seemingly the most redundant. Emora and Blender+Decode express a high rate of topic switching, with about 3 out of every 10 utterances being a topic switch. In other words, these 2 bots spend on average only 3 turns talking on a single topic before introducing a new topic. On the other hand, BART-FiDRAG and Blender2 spend more time following-up on previous ideas in the conversation rather than switching to a new topic, with nearly 6 out of 10 utterances categorized as follow-ups. Topic switching itself is not necessarily a mistake, as there are many cases in which the current discussion in a conversation wraps up so it is natural to move on, but topic switching too often can feel abrupt and cause users to feel ignored. However, given that Emora and Blender+Decode also suffer more frequently from producing irrelevant responses than the others, approaching 2 out of every 10 being irrelevant, this does suggest that their higher rate of topic switching is most likely undesirable.

==> old_latex_files/old_sections/bot-selection.tex <==
\section{Bot Selection}
\label{model_selection}

We collected a dataset of human-bot conversations from a diverse range of state-of-the-art approaches to dialogue in order to represent different aspects of conversational capabilities. To this end, we identified 4 focal themes of dialogue work in the recent literature from which we select dialogue models: general purpose, knowledge-grounded, empathy, and consistency. For each of the 4 themes, we conducted a literature review with the goal of identifying candidate dialogue models to use in our study. The criteria we used for candidate identification is as follows:

\begin{enumerate}
    \item The model must convincingly demonstrate state-of-the-art performance in a task related to the theme.
    \item The model implementation must be provided with either a trained English version available or straightforward procedure to replicate the trained model for English
    \item The response latency must be bearable (<10 seconds), on average, on modern GPU hardware.
\end{enumerate}

Once the candidate dialogue models were selected, we ran a bot pilot using members of our lab to perform a dialogue system verification check. This dialogue system verification check aimed to identify any dialogue approaches that were unable to perform as multi-turn conversational partners. Since the goal of this study is to improve the evaluation methodology of dialogue systems, it is important for the utilized models to have a baseline level of back-and-forth conversational competency. As many recent dialogue works do not evaluate their proposed approaches in such a manner - instead relying on static single turn evaluation procedures - this bot pilot enabled the filtering of insufficient dialogue approaches. 

Participants in the bot pilot connected to a custom interactive, text-based web interface from ParlAI\footnote{\href{https://parl.ai/}{https://parl.ai/}} in which they were paired with a random dialogue model. They were able to reconnect and chat with another dialogue model multiple times. At the end of each conversation, they were asked to rate the overall Quality of their conversation on a scale of 1 to 5. We used the average Quality ratings received by each model to determine which models passed the verification check. Any models that received an average rating of 3.0 or lower were considered to fail the verification check of their dialogue system suitability, if a manual review of their conversations confirmed their low rating was due to glaring and consistent response issues.

For each candidate model included in the pilot, a brief overview of the implementation details required to use them as interactive models in this work is described below:

\paragraph{Emora}
We implement a ParlAI agent using the interactive chatting mode provided for the Emora system \cite{Finch:20b}.

\paragraph{BART-FiDRAG}
An interactive chatting mode for BART-FiDRAG is provided through ParlAI. We use the default arguments, except for \texttt{compressed-indexer-nprobe} and \texttt{beam-context-block-ngram} which we set to 128 and 3, respectively, following internal testing by the authors before the pilot.

\paragraph{Blender2}
An interactive chatting mode for Blender2\footnote{\href{https://parl.ai/projects/blenderbot2/}{https://parl.ai/projects/blenderbot2/}} is provided through ParlAI; however, the internet-search augmented functionality as described in \citep{Komeili:22} is not provided. Although there is an available alternative internet search server\footnote{\href{https://github.com/JulesGM/ParlAI_SearchEngine}{https://github.com/JulesGM/ParlAI\_SearchEngine}} that is compatible with Blender2, it increased the response latency of Blender2 such that it no longer met Criteria 3. As a result, we use the version of Blender2 that does not include the internet search functionality.

\paragraph{(Blender/Blender2)+DECODE}
We implement two custom agents in the Parlai framework following the best-performing setup of \citep{Nie:21} of finetuning a consistency classification model and using it to rerank generated responses from Blender \cite{Roller:20} (or Blender2) such that the least contradictory response is selected.

\paragraph{DukeNet}
The published code for DukeNet is missing an interactive chatting mode, although a trained model on the multi-topic Wizard of Wikipedia (WoW) \cite{Dinan:18} is provided. We modified the published code to support an interactive chatting mode. However, one major difference is that the relevant knowledge documents need to be retrieved in interactive chatting mode, whereas they are predetermined in the training and evaluation environments. To remedy this, we use a trained Dense Passage Retrieval model \cite{Karpukhin:20} provided through Sentence-Transformers\footnote{\href{https://www.sbert.net/docs/pretrained-models/dpr.html}{https://www.sbert.net/docs/pretrained-models/dpr.html}} to select knowledge at each dialogue turn. We implement a ParlAI agent using the available DukeNet model and our custom interactive chatting mode.

\paragraph{CEM}
The published code for CEM is missing both an interactive chatting mode and a trained model. We trained a CEM model using the default arguments from the repository and modified the published code to support an interactive chatting mode. We implement a ParlAI agent using this trained model and our custom interactive chatting mode. 
\LN

\noindent The final selection of chatbots based on the results of the bot pilot is shown in Table \ref{tab:bot_pilot_results}. It is clear to see that several models received Likert ratings that indicated their failure as a dialogue system. Specifically, the models CEM and DukeNet failed to pass the bot pilot. DukeNet frequently produced nonsensical responses within the conversations, rendering it an ineffective conversation partner. On the other hand, CEM produced highly generic responses that merely served as reactions to the previous utterance from the user and contributed no content to the conversation itself. As a result, these models are not included in the remainder of this study. In addition, we chose to exclude the Blender2+DECODE model in favor of the higher-performing Blender+DECODE as they were two versions of the same underlying dialogue approach.

\begin{table}[htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|c}
\textbf{Model} & \textbf{Theme} & \textbf{Quality} & \textbf{N} & \textbf{Passed} \\ \hline
Blender+DECODE & Consistency & 4.100 & 10 & \cmark         \\ \hline
Blender2 & General & 3.800  & 10 & \cmark \\ \hline
BART-FiDRAG & Knowledge & 3.500 & 10 & \cmark \\ \hline
Emora & General & 3.300 & 10 & \cmark \\ \hline
Blender2+DECODE & Consistency & 2.800  & 10 & \xmark \\ \hline
DukeNet & Knowledge & 1.889 & 9 & \xmark \\ \hline
CEM & Empathy & 1.083 & 12 & \xmark \\       
\end{tabular}%
}
\caption{The bot pilot results for 7 bots, showing the theme of the approach (\textbf{Theme}), number of collected conversations (\textbf{N}), and the average (\textbf{Quality}) dialogue-level Likert quality rating per bot. The final column (\textbf{Passed}) denotes which models passed the verification criteria and were included into the full study.}
\label{tab:bot_pilot_results}
\end{table}





==> old_latex_files/old_sections/evaluation-analysis.tex <==
\section{Evaluation Metric Assessment}

\subsection{Predictive Validity}

\begin{figure}[ht]
\centering
\includegraphics[width=\columnwidth]{tex/fig/pred_validity.png}
\caption{Amount of variance in conversation quality  captured from each evaluation metric.}
\label{fig:predictive_validity}
\end{figure}

To show the relative importance of each metric with respect to explaining dialogue quality, we present a univariate regression analysis for each of our labels. Each regression model $R_l$ for label $l$ is fit to a set of $(X_{li}, Y_{i})$ pairs, where each $X_{li}$ is the metric measurement of label $l$ for conversation $i$, and each $Y_{i}$ is a quality measurement for that conversation. In the presented analysis (\ref{fig:predictive_validity}), we use all 400 conversations to fit each regression model. The static dialogue likert quality labels are used as the quality outcome metric $Y$ for each dialogue. Since this metric is ordinal in nature, but often approximated as ratio data, we show results for fitting both linear and ordinal regression models. 

\subsection{Incremental Validity}

Here we investigate the coverage of each of our labels with respect to explaining conversation quality. To determine the extent that each label provides new information about conversation quality above and beyond other labels, we perform a stepwise regression analysis. Similar to the previous subsection, we use our static dialogue likert quality labels as the target outcome and every other non-quality metric as features.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{tex/fig/inc_validity.png}
%     \caption{Incremental validity results. TODO - increase font size of labels, reposition labels, add legend}
%     \label{fig:my_label}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{tex/fig/inc_validity_small.png}
    \caption{Incremental validity results. TODO - increase font size of labels, reposition labels, add legend}
    \label{fig:my_label}
\end{figure}


% % generated using https://www.tablesgenerator.com/latex_tables#
% \begin{table}[htbp]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|ll|ll|ll|}
% \hline
% \multicolumn{2}{|c|}{\textbf{ABC-Eval}} & \multicolumn{2}{c|}{\textbf{Likert Turn}} & \multicolumn{2}{c|}{\textbf{Likert Dialogue}} \\ \hline
% \multicolumn{1}{|l|}{antisocial} & 15.9640 (nan) & \multicolumn{1}{l|}{grammatical} & 8.5660 (nan) & \multicolumn{1}{l|}{emotional} & 58.4260 (nan) \\ \hline
% \multicolumn{1}{|l|}{life info} & 15.9550 (-0.0090) & \multicolumn{1}{l|}{informative} & 8.5080 (-0.0580) & \multicolumn{1}{l|}{informative} & 57.8320 (-0.5940) \\ \hline
% \multicolumn{1}{|l|}{preference info} & 15.8500 (-0.1050) & \multicolumn{1}{l|}{engaging} & 8.2850 (-0.2230) & \multicolumn{1}{l|}{grammatical} & 56.4390 (-1.3930) \\ \hline
% \multicolumn{1}{|l|}{commonsense contradiction} & 15.6920 (-0.1580) & \multicolumn{1}{l|}{emotional} & 7.7530 (-0.5320) & \multicolumn{1}{l|}{relevant} & 54.5170 (-1.9220) \\ \hline
% \multicolumn{1}{|l|}{uninterpretable} & 15.5030 (-0.1890) & \multicolumn{1}{l|}{consistent} & 6.8890 (-0.8640) & \multicolumn{1}{l|}{proactive} & 51.6360 (-2.8810) \\ \hline
% \multicolumn{1}{|l|}{ignore} & 15.2500 (-0.2530) & \multicolumn{1}{l|}{proactive} & 5.7860 (-1.1030) & \multicolumn{1}{l|}{consistent} & 48.6730 (-2.9630) \\ \hline
% \multicolumn{1}{|l|}{correct fact} & 15.1970 (-0.0530) & \multicolumn{1}{l|}{relevant} & 3.7760 (-2.0100) & \multicolumn{1}{l|}{engaging} & 38.1030 (-10.5700) \\ \hline
% \multicolumn{1}{|l|}{topic switch} & 14.8090 (-0.3880) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{follow up} & 14.5270 (-0.2820) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{redundant} & 14.3660 (-0.1610) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{lack of empathy} & 13.9250 (-0.4410) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{incorrect fact} & 13.5470 (-0.3780) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{self contradiction} & 12.6080 (-0.9390) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{irrelevant} & 11.0490 (-1.5590) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{empathetic} & 9.4890 (-1.5600) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \multicolumn{1}{|l|}{partner contradiction} & 6.0430 (-3.4460) & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  \\ \hline
% \end{tabular}%
% }
% \caption{The results for the incremental validity procedure on each evaluation. The R-squared value for a particular row results from the model fit on all labels up to and including that row from bottom-to-top. The value in parenthesis indicates the gain in R-squared from the previous model (i.e. the previous row).}
% \label{tab:inc_validity}
% \end{table}


\subsection{Evaluation Sensitivity}

The metric variance is relative to the variance in the underlying metric distribution across the bot population. Unfortunately, we do not have a large random sample of bots in this work, so to answer the question of evaluation metric sensitivity we present a case study of the evaluations' abilities to detect differences between the 4 bots we selected. 

\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l | c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c }

\textbf{Label} & \rot{$\sim$Soc$_b$} & \rot{$\sim$Com$_b$} & \rot{Fac$_b$} & \rot{Emp$_b$} & \rot{Fol$_b$} & \rot{Ign$_b$} & \rot{$\sim$Fac$_b$} & \rot{$\sim$Rel$_b$} & \rot{$\sim$Emp$_b$} & \rot{Lif$_b$} & \rot{$\sim$Par$_b$} & \rot{Pre$_b$} & \rot{Red$_b$} & \rot{$\sim$Sel$_b$} & \rot{Top$_b$} & \rot{$\sim$Int$_b$} & \rot{Con$_t$} & \rot{Emo$_t$} & \rot{Eng$_t$} & \rot{Gra$_t$} & \rot{Inf$_t$} & \rot{Pro$_t$} & \rot{Qua$_t$} & \rot{Rel$_t$}  & \rot{Con$_d$} & \rot{Emo$_d$} & \rot{Eng$_d$} & \rot{Gra$_d$} & \rot{Inf$_d$} & \rot{Pro$_d$} & \rot{Qua$_d$} & \rot{Rel$_d$} & \rot{Con$_c$} & \rot{Emo$_c$} & \rot{Eng$_c$} & \rot{Gra$_c$} & \rot{Inf$_c$} & \rot{Pro$_c$} & \rot{Qua$_c$} & \rot{Rel$_c$}  \\ \hline
0.01 & 0 & 1 & 4 & 3 & 5 & 1 & 4 & 2 & 4 & 2 & 0 & 4 & 2 & 5 & 5 & 2 & 1 & 1 & 2 & 4 & 4 & 4 & 4 & 2 & 1 & 2 & 1 & 0 & 0 & 3 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 1 & 0 & 0 \\
0.05 & 0 & 2 & 5 & 3 & 5 & 2 & 6 & 2 & 5 & 2 & 1 & 4 & 3 & 5 & 5 & 3 & 2 & 1 & 3 & 5 & 4 & 4 & 4 & 3 & 2 & 3 & 2 & 3 & 2 & 3 & 1 & 2 & 1 & 0 & 1 & 0 & 1 & 2 & 1 & 0 \\
0.1 & 1 & 3 & 5 & 3 & 5 & 2 & 6 & 2 & 5 & 3 & 1 & 4 & 3 & 5 & 5 & 3 & 2 & 3 & 3 & 5 & 4 & 4 & 4 & 4 & 2 & 4 & 2 & 5 & 3 & 3 & 3 & 2 & 2 & 0 & 1 & 0 & 2 & 2 & 1 & 2
\end{tabular}%
}
\caption{The number of bot pairs that are significantly different from one another based on 32 annotated conversations with regard to the evaluation label at three sensitivity levels (0.01, 0.05, 0.1). The maximum value for any entry is 6 as there are 6 bot-pairs in this work.}
\label{tab:sensivity}
\end{table*}


\subsection{Evaluation Cost Analysis}

Table \ref{tab:costs}\input{tex/excerpts/costs.tex}

\begin{table}[htbp]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\textbf{Evaluation} & \textbf{Median Time} & \textbf{Throughput} & \textbf{Estimated Cost} & \textbf{Our Cost}  \\ \hline \hline
Likert Dialogue & 2.81 & 21.37 & 374.36 & 240.00  \\ \hline
Comparative & 4.35 & 13.81 & 289.68 & 286.67  \\ \hline
Likert Turn & 19.94 & 3.01 & 2658.40 & 2240.00  \\ \hline
ABC-Eval & 25.60 & 2.34 & 3413.58 & 3422.67 \\ 
\end{tabular}%
}
\caption{The costs incurred for each evaluation procedure. \textbf{Median Time} is the median completion time in minutes to annotate one dialogue by a Surge annotator. \textbf{Throughput} is the number of fully annotated dialogues that can be produced by a single annotator in one hour. \textbf{Projected Cost} is the estimated cost to fully annotate 400 dialogues at a rate of \$20 per hour using the median completion time. \textbf{Our Cost} is the total amount paid in this work to collect 400 fully singly annotated conversations. }
\label{tab:costs}
\end{table}





==> old_latex_files/old_sections/evaluation-collection.tex <==
\section{Evaluation Collection}
\label{sec:annotation-collection}

Once the 400 human-bot conversations were collected, we collected annotations according to all 4 of the identified evaluation procedures under study as described below. Subscripts denote evaluation type hereafter.

\paragraph{Behavior$_b$} 8 annotation tasks were performed for the Behavior evaluation procedure, following the procedure described in \sref{sec:behavior-evaluation}. \LN

\noindent For each of the remaining evaluation procedures, 8 annotation tasks were performed, following the 8 human dimensions of evaluation identified in \cite{Finch:20}. Shorthand tags (Table \ref{tab:dims}) are used hereafter to refer to specific dimensions.

\begin{table}[htbp!]
\centering
  \begin{small}
  \begin{tabular}{ l | l }

  \bf Dimension & \bf Tag \\
  \hline \hline
  Grammaticality & \tt Gra \\
  \hline
  Relevance & \tt Rel \\
  \hline
  Informativeness & \tt Inf \\
  \hline
  Emotional Understanding & \tt Emo  \\
  \hline
  Engagingness & \tt Eng \\
  \hline
  Consistency & \tt Con \\
  \hline
  Proactivity & \tt Pro \\
  \hline
  Quality & \tt Qua \\

  \end{tabular}
  \end{small}
  
  \caption{Shorthand tags of the 8 dimensions}
  \label{tab:dims}
\end{table}

\paragraph{Dialogue Likert$_d$} For each dimension, the annotator was presented with the conversation and a description of the dimension under consideration. Given this information, their task was to select the rating on a 1 - 5 Likert scale that holistically represents the conversation with respect to the dimension.

\paragraph{Turn Likert$_t$} For each dimension, the annotator was presented with the conversation and a description of the dimension under consideration. For each turn of the conversation, their task was to select the rating on a 1 - 5 Likert scale that appropriately represents the turn with respect to the dimension.

\paragraph{Comparative$_c$} For each dimension, the annotator was presented with two conversations and a description of the dimension under consideration. Given this information, their task was to select which conversation was better with respect to the dimension. The annotators were allowed to indicate that neither conversation was better, but they were instructed to use this only as a last resort. \LN

\noindent For each annotation task, 108 conversations were annotated by two annotators while the remaining 292 conversations were annotated by one annotator.

\subsection{Annotator Qualification}
\label{sec:workforces}

One important consideration when performing evaluations is the selection of the annotator group. After review of recent works on dialogue approaches, there is not one obvious standard for how to obtain dialogue evaluation annotations. Indeed, three possible sources of human annotators were identified: 

\paragraph{Recruitment} Annotators were recruited participants, often from the student population at the author's academic institution.

\paragraph{Crowdsourcing} The annotation work was published on a crowdsourcing platform from which workers could take assignments. The most common crowdsourcing platform to use is Amazon Mechanical Turk.

\paragraph{Third-party} The annotation work was conducted in collaboration with a hired third-party company, which provides a dedicated workforce. \LN

\noindent In order to determine the best-fitting group for the annotation collection, we investigated the viability of each. We published annotations tasks to the recruited students in \sref{sec:conversation-collection}, the Amazon Mechanical Turk platform\footnote{\href{https://www.mturk.com/}{https://www.mturk.com/}}, and the Surge platform\footnote{\href{https://www.surgehq.ai/}{https://www.surgehq.ai/}} as the three groups, respectively. 

Overall, only one group of annotators was found to be a viable method for collecting the quantity of annotations required for this study - the third-party platform Surge - due to their high work throughput and diligence on learning to perform well on the annotation tasks. In one week, students completed 343 assignments, Mturkers completed 56 assignments and Surgers completed 2032 assignments. Overall, the training pass rates for each group can be found in Figure \ref{fig:training_rates}. The student group displayed the necessary diligence, but did not have the willingness to provide the quantity of work needed. The Mturk group was neither diligent enough to be accurate in their annotations nor willing to complete the tasks in a timely manner.

% \begin{table}[htbp]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|l|l|l}
%  & \textbf{Students} & \textbf{MTurk} & \textbf{Surge} \\ \hline
% \textbf{Dialogue Likert} & 15 & 5 & 400 \\ \hline
% \textbf{Turn Likert} & 13.75 & 4 & 400 \\ \hline
% \textbf{Comparative} & 12 & 5 & 202 \\ \hline
% \textbf{Behavior} & 8.5 & 4 & 400
% \end{tabular}%
% }
% \caption{The average number of tasks completed by each annotation workforce across all annotation tasks for each evaluation procedure.}
% \label{tab:completion_rates}
% \end{table}

% \begin{table}[htbp]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|l|l|l}
%  & \textbf{Students} & \textbf{MTurk} & \textbf{Surge} \\ \hline
% \textbf{Interpretability} & 0.75 (9/12) & 0.64 (7/11) & 0.88 (22/25) \\ \hline
% \textbf{Personal Information} & 0.69 (9/13) & 0.36 (4/11) & 0.75 (24/32) \\ \hline
% \textbf{Knowledge} & 0.88 (7/8) & 0.31 (4/13) & 0.86 (25/29) \\ \hline
% \textbf{Empathy} & 0.67 (10/15) & 0.18 (5/28) & 0.58 (18/31) \\ \hline
% \textbf{Commonsense} & 0.89 (8/9) & 0.83 (5/6) & 0.91 (20/22) \\ \hline
% \textbf{Sociality} & 1.00 (7/7) & 0.71 (5/7) & 1.00 (14/14) \\ \hline
% \textbf{Consistency} & 1.00 (5/5) & 0.19 (6/32) & 0.62 (13/21) \\ \hline
% \textbf{Transitions} & 1.00 (5/5) & 0.00 (0/24) & 0.41 (22/54)
% \end{tabular}%
% }
% \caption{The training pass rate of each annotation workforce for the behavior evaluation tasks. Each cell displays the proportion of annotators who passed the training, with the number of passed and the total number of attempts shown in parenthesis.}
% \label{tab:pass_rates}
% \end{table}

\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{tex/fig/training_rates.png}
\caption{The training pass rate of each annotation work-
force for the behavior evaluation tasks.}
\label{fig:training_rates}
\end{figure}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=\columnwidth]{tex/fig/worker_completions.png}
% \caption{The number of assignments completed by each annotation work-force over time.}
% \label{fig:worker_completions}
% \end{figure}


\subsection{Annotation Agreements}

It is necessary for there to be relatively high annotator agreement on evaluation tasks to ensure the reliability and quality of the resultant comparisons. Interannotator agreements indicated by Krippendorf's alpha (CITE) were calculated for each label within each evaluation methodology using the 108 doubly-annotated conversations. As shown in Figure \ref{fig:surge_agreement}, existing evaluation procedures produce mediocre interannotator agreements, rarely achieving agreement higher than 0.4. ABC-Eval achieves much higher agreement, with most labels achieving agreements greater than 0.4, and several nearing agreements of 0.6 or higher.

Within ABC-Eval, the labels \texttt{antisocial} and \texttt{uninterpretable} were outliers in terms of variance and agreement, respectively. Current state-of-the-art chatbots rarely produce these behaviors, thus resulting in very few positive cases. Most agreement metrics - including Krippendorf's alpha - incorporate a measure of expectation when calculating agreement. In cases of highly imbalanced ground-truth 
annotation rates, this results in low agreement scores even if the majority of annotations agree on the negative label.   

Interestingly, there is no clear evidence that a Comparative approach to dialogue evaluation is more reliable or produces better annotator agreement than a Likert approach, as claimed in previous works (CITE acute eval, beyond likert ratings). Instead, both seem to produce similar agreement distributions, with comparable variance.

The results do suggest that turn-based evaluation procedures are able to produce less variable agreements, as shown by the tight confidence intervals. However, this can be explained by the multiplicative effect on the sample size of the turn-based approach; each dialogue becomes N times as many datapoints depending on the turn length, rather than just a single datapoint as for dialogue-level evaluation procedures like Dialogue Likert and Dialogue Comparative. Even so, this does suggest that
a lower dialogue collection cost can be endured without sacrificing reliability of the resultant annotations for turn-based evaluation procedures.


% For each label type (including all behavior labels, all likert labels, all comparative labels), show agreements (Fleiss Kappa, Cripp Alpha, Kend Tau) for students, mturkers, surgers, and experts (table??). Takeaway: behavior labels have good agreement for subjectivity of task, and have overall higher agreement than likert and comparative labels.

% For each label type (all), show agreements (Fleiss Kappa, Cripp Alpha, Kend Tau) for students (interactive), students (static), mturkers, and surgers against experts. Takeaway: high agreement with experts indicates the annotations measure what the authors intend, low agreement indicates that the guideline has bias that does not reflect the author's intention.

% (Problem: the above tables are probably too large, how to present more elegantly?)

\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{tex/fig/surge_agreement.png}
\caption{Interannotator agreements for Surge workforce on all dialogue evaluation metrics. Error bars denote 95\% confidence interval of interannotator agreement.}
\label{fig:surge_agreement}
\end{figure}

% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l|l|l|l}
% category & label & $\alpha$ & CI low & CI high & $\kappa$ & CI low.1 & CI high.1 & n \\ \hline
% likert turn & grammatical & 0.419 & 0.372 & 0.464 & 0.296 & 0.259 & 0.333 & 1634 \\ \hline
% likert turn & quality & 0.312 & 0.267 & 0.357 & 0.092 & 0.061 & 0.122 & 1634 \\ \hline
% likert turn & engaging & 0.295 & 0.246 & 0.344 & 0.123 & 0.092 & 0.153 & 1634 \\ \hline
% likert turn & proactive & 0.279 & 0.232 & 0.327 & 0.098 & 0.071 & 0.125 & 1634 \\ \hline
% likert turn & informative & 0.278 & 0.233 & 0.321 & 0.092 & 0.065 & 0.123 & 1634 \\ \hline
% likert turn & relevant & 0.239 & 0.190 & 0.287 & 0.100 & 0.068 & 0.132 & 1634 \\ \hline
% likert turn & consistent & 0.201 & 0.150 & 0.252 & 0.083 & 0.052 & 0.116 & 1634 \\ \hline
% likert turn & emotional & 0.166 & 0.119 & 0.214 & 0.021 & -0.009 & 0.056 & 1634 \\ \hline
% likert dialogue & informative & 0.409 & 0.257 & 0.531 & 0.031 & -0.089 & 0.157 & 108 \\ \hline
% likert dialogue & consistent & 0.360 & 0.199 & 0.511 & 0.074 & -0.023 & 0.202 & 108 \\ \hline
% likert dialogue & relevant & 0.298 & 0.133 & 0.455 & -0.003 & -0.105 & 0.126 & 108 \\ \hline
% likert dialogue & quality & 0.286 & 0.117 & 0.452 & 0.078 & -0.028 & 0.205 & 108 \\ \hline
% likert dialogue & engaging & 0.259 & 0.074 & 0.435 & 0.123 & 0.007 & 0.265 & 108 \\ \hline
% likert dialogue & emotional & 0.256 & 0.082 & 0.433 & 0.046 & -0.057 & 0.178 & 108 \\ \hline
% likert dialogue & proactive & 0.243 & 0.040 & 0.426 & -0.026 & -0.121 & 0.079 & 108 \\ \hline
% likert dialogue & grammatical & 0.132 & -0.033 & 0.297 & -0.058 & -0.173 & 0.082 & 108 \\ \hline
% comparative & consistent & 0.484 & 0.318 & 0.629 & 0.481 & 0.308 & 0.645 & 108 \\ \hline
% comparative & quality & 0.447 & 0.283 & 0.631 & 0.444 & 0.295 & 0.611 & 108 \\ \hline
% comparative & relevant & 0.418 & 0.238 & 0.578 & 0.392 & 0.226 & 0.553 & 108 \\ \hline
% comparative & proactive & 0.226 & 0.058 & 0.391 & 0.222 & 0.037 & 0.425 & 108 \\ \hline
% comparative & grammatical & 0.215 & 0.050 & 0.390 & 0.024 & -0.088 & 0.162 & 108 \\ \hline
% comparative & informative & 0.209 & 0.031 & 0.379 & 0.200 & 0.027 & 0.382 & 108 \\ \hline
% comparative & emotional & 0.202 & 0.016 & 0.387 & 0.074 & -0.050 & 0.209 & 108 \\ \hline
% comparative & engaging & 0.115 & -0.052 & 0.300 & 0.111 & -0.069 & 0.302 & 108 \\ \hline
% behavior & topic switch & 0.755 & 0.714 & 0.795 & 0.755 & 0.715 & 0.791 & 1634 \\ \hline
% behavior & incorrect fact & 0.652 & 0.570 & 0.717 & 0.651 & 0.577 & 0.711 & 1634 \\ \hline
% behavior & life info & 0.631 & 0.588 & 0.676 & 0.631 & 0.586 & 0.672 & 1634 \\ \hline
% behavior & correct fact & 0.618 & 0.570 & 0.660 & 0.618 & 0.569 & 0.664 & 1634 \\ \hline
% behavior & ignore & 0.571 & 0.502 & 0.630 & 0.571 & 0.500 & 0.632 & 1634 \\ \hline
% behavior & antisocial & 0.553 & 0.220 & 0.799 & 0.553 & 0.231 & 0.823 & 1634 \\ \hline
% behavior & redundant & 0.551 & 0.470 & 0.624 & 0.551 & 0.477 & 0.623 & 1634 \\ \hline
% behavior & empathetic & 0.514 & 0.472 & 0.558 & 0.513 & 0.475 & 0.556 & 1634 \\ \hline
% behavior & follow up & 0.492 & 0.447 & 0.533 & 0.492 & 0.447 & 0.532 & 1634 \\ \hline
% behavior & preference info & 0.491 & 0.449 & 0.532 & 0.491 & 0.446 & 0.536 & 1634 \\ \hline
% behavior & irrelevant & 0.456 & 0.396 & 0.511 & 0.456 & 0.396 & 0.516 & 1634 \\ \hline
% behavior & commonsense contradiction & 0.442 & 0.387 & 0.493 & 0.442 & 0.390 & 0.496 & 1634 \\ \hline
% behavior & partner contradiction & 0.436 & 0.365 & 0.514 & 0.436 & 0.363 & 0.509 & 1634 \\ \hline
% behavior & lack of empathy & 0.435 & 0.376 & 0.497 & 0.435 & 0.369 & 0.493 & 1634 \\ \hline
% behavior & self contradiction & 0.407 & 0.321 & 0.504 & 0.406 & 0.316 & 0.494 & 1634 \\ \hline
% behavior & uninterpretable & 0.137 & 0.031 & 0.299 & 0.137 & 0.029 & 0.293 & 1634 \\ \hline
% \end{tabular}%
% }
% \caption{Interannotator agreements for Surge workforce on all dialogue evaluation metric. Krippendorf's alpha: $\alpha$, Fleiss' kappa: $\kappa$}
% \label{tab:surge_agreements}
% \end{table*}

% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l|l|l|l}
% category & label & $\alpha$ & CI low & CI high & $\kappa$ & CI low.1 & CI high.1 & n \\ \hline
% likert turn & proactive & 0.254 & 0.027 & 0.453 & 0.075 & -0.051 & 0.249 & 75 \\ \hline
% likert turn & consistent & 0.185 & -0.063 & 0.385 & -0.097 & -0.202 & 0.070 & 75 \\ \hline
% likert turn & quality & 0.001 & -0.220 & 0.235 & 0.047 & -0.067 & 0.184 & 75 \\ \hline
% likert turn & grammatical & -0.032 & -0.210 & 0.160 & -0.200 & -0.254 & -0.098 & 75 \\ \hline
% likert turn & emotional & -0.036 & -0.235 & 0.183 & 0.040 & -0.074 & 0.202 & 75 \\ \hline
% likert turn & informative & -0.113 & -0.324 & 0.111 & -0.005 & -0.099 & 0.127 & 75 \\ \hline
% likert turn & engaging & -0.171 & -0.350 & 0.067 & -0.088 & -0.181 & 0.060 & 75 \\ \hline
% likert turn & relevant & -0.208 & -0.410 & 0.055 & -0.002 & -0.118 & 0.157 & 75 \\ \hline
% likert dialogue & quality & 0.635 &  &  & -0.111 & -0.613 & 0.412 & 5 \\ \hline
% likert dialogue & consistent & 0.567 & -0.605 & 0.986 & 0.211 & -0.250 & 1.000 & 5 \\ \hline
% likert dialogue & engaging & 0.540 &  &  & -0.034 &  &  & 5 \\ \hline
% likert dialogue & relevant & 0.383 & -0.800 & 0.943 & 0.032 & -1.000 & 0.655 & 5 \\ \hline
% likert dialogue & grammatical & 0.327 &  &  & 0.091 &  &  & 5 \\ \hline
% likert dialogue & proactive & 0.100 & -0.043 & 0.100 & -0.429 &  &  & 5 \\ \hline
% likert dialogue & emotional & 0.068 & -0.800 & 0.068 & -0.613 & -1.000 & -0.613 & 5 \\ \hline
% likert dialogue & informative & -0.500 &  &  & -0.212 & -0.613 & 0.286 & 5 \\ \hline
% comparative & proactive & 0.688 & 0.258 & 0.981 & 0.238 & -0.143 & 0.775 & 8 \\ \hline
% comparative & emotional & 0.531 &  &  & 0.500 & -0.270 & 1.000 & 8 \\ \hline
% comparative & informative & 0.531 &  &  & 0.500 & -0.333 & 1.000 & 8 \\ \hline
% comparative & engaging & 0.330 & -0.354 & 0.933 & 0.169 & -0.352 & 0.768 & 8 \\ \hline
% comparative & relevant & 0.330 & -0.470 & 0.911 & 0.169 & -0.349 & 0.768 & 8 \\ \hline
% comparative & grammatical & 0.062 & -0.500 & 0.762 & 0.000 & -0.600 & 0.746 & 8 \\ \hline
% comparative & consistent & -0.205 & -0.671 & 0.519 & -0.247 & -0.580 & 0.488 & 8 \\ \hline
% comparative & quality & -0.205 & -0.671 & 0.548 & -0.247 & -0.600 & 0.376 & 8 \\ \hline
% behavior & redundant & 0.687 & 0.247 & 0.916 & 0.685 & 0.220 & 0.916 & 75 \\ \hline
% behavior & commonsense contradiction & 0.567 & -0.017 & 0.924 & 0.564 & -0.006 & 0.914 & 60 \\ \hline
% behavior & correct fact & 0.567 & 0.321 & 0.751 & 0.564 & 0.322 & 0.755 & 75 \\ \hline
% behavior & incorrect fact & 0.553 &  &  & 0.550 &  &  & 75 \\ \hline
% behavior & self contradiction & 0.539 & 0.149 & 0.803 & 0.536 & 0.173 & 0.801 & 75 \\ \hline
% behavior & partner contradiction & 0.444 & 0.100 & 0.771 & 0.440 & 0.056 & 0.747 & 75 \\ \hline
% behavior & empathetic & 0.385 & -0.073 & 0.764 & 0.375 & -0.118 & 0.760 & 30 \\ \hline
% behavior & life info & 0.352 & -0.019 & 0.660 & 0.346 & 0.020 & 0.677 & 60 \\ \hline
% behavior & preference info & 0.248 & -0.037 & 0.558 & 0.242 & -0.028 & 0.545 & 60 \\ \hline
% behavior & antisocial & 0.000 &  &  & -0.007 &  &  & 75 \\ \hline
% behavior & lack of empathy & -0.073 &  &  & -0.091 &  &  & 30 \\ \hline
% behavior & uninterpretable &  &  &  &  &  &  & 75 \\ \hline
% \end{tabular}%
% }
% \caption{Interannotator agreements for MTurk workforce on all dialogue evaluation metric. Krippendorf's alpha: $\alpha$, Fleiss' kappa: $\kappa$}
% \label{tab:mturk_agreements}
% \end{table*}

% \begin{table*}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l|l|l|l}
% category & label & $\alpha$ & CI low & CI high & $\kappa$ & CI low.1 & CI high.1 & n \\ \hline
% likert turn & grammatical & 0.220 & 0.100 & 0.336 & 0.092 & 0.014 & 0.185 & 368 \\ \hline
% likert turn & relevant & -0.163 & -0.242 & -0.070 & -0.081 & -0.132 & -0.011 & 368 \\ \hline
% likert turn & informative & -0.491 & -0.573 & -0.398 & -0.224 & -0.269 & -0.165 & 368 \\ \hline
% likert dialogue & informative & 0.627 &  &  & 0.316 & -0.162 & 0.798 & 10 \\ \hline
% likert dialogue & consistent & 0.557 & 0.117 & 0.874 & 0.077 & -0.314 & 0.585 & 10 \\ \hline
% likert dialogue & proactive & 0.402 & 0.041 & 0.855 & 0.070 & -0.359 & 0.688 & 10 \\ \hline
% likert dialogue & engaging & 0.328 & -0.095 & 0.745 & -0.138 & -0.513 & 0.487 & 10 \\ \hline
% likert dialogue & grammatical & 0.268 & -0.462 & 0.798 & -0.053 & -0.538 & 0.478 & 10 \\ \hline
% likert dialogue & relevant & 0.256 & -0.727 & 0.789 & -0.102 & -1.000 & 0.375 & 10 \\ \hline
% likert dialogue & quality & 0.228 & -0.387 & 0.781 & 0.055 & -0.364 & 0.644 & 10 \\ \hline
% likert dialogue & emotional & 0.182 & -0.410 & 0.634 & -0.094 & -0.417 & 0.479 & 10 \\ \hline
% comparative & consistent & 0.681 & 0.148 & 1.000 & 0.667 & 0.111 & 1.000 & 12 \\ \hline
% comparative & engaging & 0.681 & 0.398 & 0.911 & 0.238 & -0.143 & 0.678 & 12 \\ \hline
% comparative & quality & 0.681 & 0.161 & 1.000 & 0.667 & -0.005 & 1.000 & 12 \\ \hline
% comparative & grammatical & 0.564 & -0.013 & 0.925 & 0.418 & -0.024 & 0.839 & 12 \\ \hline
% comparative & proactive & 0.425 & -0.164 & 0.853 & 0.200 & -0.168 & 0.701 & 12 \\ \hline
% comparative & informative & 0.361 & -0.193 & 0.839 & 0.333 & -0.175 & 0.832 & 12 \\ \hline
% comparative & relevant & 0.361 & -0.178 & 0.839 & 0.333 & -0.244 & 0.832 & 12 \\ \hline
% comparative & emotional & 0.216 & -0.315 & 0.799 & 0.127 & -0.274 & 0.678 & 12 \\ \hline
% behavior & uninterpretable & 0.322 &  &  & 0.320 &  &  & 152 \\ \hline
% behavior & antisocial &  &  &  &  &  &  & 233
% \end{tabular}%
% }
% \caption{Interannotator agreements for Student workforce on all dialogue evaluation metric. Krippendorf's alpha: $\alpha$, Fleiss' kappa: $\kappa$}
% \label{tab:student_agreements}
% \end{table*}




==> old_latex_files/old_sections/human-bot-interaction.tex <==
\section{Human-to-Bot Interaction}
\label{sec:conversation-collection}

% Description of student participants (undergrads, major distribution, compensation)

% Collection setting description (chat tool, blindness, instructions given, reps per person, interactive annotations)

For our evaluation and analysis, we collected 400 conversations between the 4 verified chatbots and human interactors, 100 with each chatbot. Human interactors were undergraduate university students recruited via email and word-of-mouth advertising in the computer science and psychology departments. 46 interactors were recruited to complete 12-18 conversations and were compensated with a \$5 Amazon gift card for every 6 completed conversations. The majority of the interactors have more than one major of study, but the most popular backgrounds include computer science (41\%), psychology (22\%), quantitative science (20\%), and linguistics (17\%). Additional details on the collected dialogues are shown in Table \ref{tab:collected_dialogue_summary}. The total cost of this conversation collection was \$333.33. 

As in our bot pilot (\sref{model_selection}), our recruits interacted with the chatbots remotely using our custom ParlAI chat interface. We emailed each interactor a set of hyperlinks to connect to the chat app in their browser, along with some brief instructions. Each time an interactor connected to the chat app, they were guided through a pair of conversations with a randomly selected two of our four chatbots. Interactors were aware they were conversing with chatbots, but had no information about what chat models they were talking with. Our instructions prompt the user to have an engaging conversation with the chatbot, but do not prescribe a specific topic or type of conversation. Since our focus is on cooperative chat, we did instruct users to avoid deliberate, unprovoked attempts to harass, insult, or quiz the chatbots. Additionally, we encouraged interactors to use correct spelling and punctuation, and to refrain from "texting language" (e.g. "lol").

Following each conversation, the interactor was instructed to rate the conversation on a randomly-ordered set of Likert scales on 8 dialogue dimensions. At the conclusion of one entire session (e.g. two conversations and two Likert rating sessions), the interactor was instructed to perform a comparative evaluation between the pair of conversations by selecting which conversation was superior on a randomly-ordered set of 8 dialogue dimensions.  We manually reviewed all collected conversations and verified that all interactors made a clear effort to follow the instructions.

\begin{table}[htbp]
\centering
\begin{tabular}{|r|l|}
\hline
Dialogues        & 400  \\ \hline
Average turns       & 30.3 \\ \hline
Average user turn length & 11.3 \\ \hline
\end{tabular}%
\caption{Summary statistics for the collected dialogues, showing the number of dialogues collected (\textbf{Dialogues}), the average number of total turns in each dialogue (\textbf{Average turns}), and the average word count of user utterances (\textbf{Average user turn length}).}
\label{tab:collected_dialogue_summary}
\end{table}






==> old_latex_files/old_sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% Novel method for human evaluation of chatbots with comparison to existing human evals

% Collection and annotation of conversations with SOTA bots to estimate prevalence and impact of various issues

State-of-the-art chatbot models still suffer from a number of issues that have been highlighted in the error analyses of recent proposed models. Problems like hallucinations, forgetfulness of context, self-contradictions, and redundancy are all still issues that are the subject of current research. Despite the prevalence of these issues, most current chatbot evaluation methods do not precisely quantify the rate of occurrence of these problems in conversations with the chatbots.

In general, it is challenging to evaluate chat-oriented dialogue.

First, variance in user preferences means that different people will have different levels of satisfaction even from the same conversation. 

Second, there are multiple ways to quantify user satisfaction as a task objective. 

A third challenge is that there are multiple facets of conversation that contribute to whether or not it is satisfying. For example, people often break down the satisfaction into dimensions such as consistency, informativeness, engagingness, etc. (CITE). The chat setting can have a significant influence on which facets are more important to users. Knowledge-grounded dialogue, for example, places heavier emphasis on the informative nature of the responses whereas persona-grounded dialogue is more focused on the chatbot's ability to express personal information in a consistent and interesting way. 

We aim to address these challenges with a novel chatbot evaluation procedure. Our proposed method involves turn-level human annotations of each chatbot response for various behaviors exhibited by the chatbot. Taking inspiration from behavioral coding methods in psychology (CITE), our evaluation encodes the rate at which a chatbot will express various phenomena such as hallucination, self-contradiction, etc. 

Binary turn-level labels have several advantages over likert- and comparative-style chatbot evaluations. First, our evaluation is subject to less variance due to differences in the individual preferences of human evaluators. This is because evaluation decisions are restricted to interpreting whether or not a particular behavior is expressed in a chatbot response, rather than asking evaluators to rate the goodness or badness of the conversation along several dimensions.
Second, the metric outcomes of evaluating a chatbot on our behavior labels are interpretable as absolute values, since each represents the percentage of the chatbot's responses that will exhibit a particular behavior (e.g. the chatbot contradicts itself 5\% of the time).

We show that this behavioral evaluation method produces fine-grained evaluation metrics that are more reliable for detecting differences in chatbot characteristics than other methods. 

Given the merits of this new methodology, we recommend that these evaluation protocols be utilized in future dialogue works in order to promote better interpretability of the successes and limitations of new approaches to chat-oriented dialogue modelling.

% https://docs.google.com/presentation/d/1IfsnmOQjQqY42243UXKVGVjC7c78zrN7w00SnzT27Xw/edit?usp=sharing
% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=\textwidth]{tex/fig/project-stages-intro-figure.png}
% \caption{Stages of Development and Validation of our Evaluation Procedure.}
% \label{fig:model}
% \end{figure*}


















==> old_latex_files/old_sections/related-work.tex <==
\section{Related Work}
\label{sec:related-work}

Integrated Taxonomy: \cite{Higashinaka:21}

\cite{Mitsuda:22} extended the taxonomy of \cite{Higashinaka:21} by targeting persona-specific errors, including \texttt{self-recognition/-relation} errors where the dialogue agent produces contradictions about its own personal information as well as \texttt{other-recognition/-relation} where the dialogue agent reveals a lack of knowledge about entities it should know according to its persona. Even though these are specific to persona-grounded agents, they can be seen as subclasses of the more general error type we include of self-contradiction.

There have been efforts to produce behavior and error coding schemes for task-oriented dialogue systems, such as customer support bots \cite{Li:20,Kvale:20,Folstad:21}. This has led to the developments of evaluation frameworks such as PARADISE \cite{Walker:97}. These frameworks often focus on dialogue efficiency, request fulfillment, and other markers of task success, which are not directly transferable to the chat-oriented dialogue systems, although more recent works include concepts such as response relevance and response understandability \cite{Folstad:21} which has applicability to the chat domain.

Dialogue Breakdown Detection works (DBDC5 had a error classification track) -- used Higashinaka 2019 according to \href{https://groups.google.com/a/wing.comp.nus.edu.sg/g/sing/c/vzTnoo7Nctg?pli=1}{this link}?

Our SIGDIAL survey: \cite{Finch:20}

Consistency, repetition, other issues, etc. as reported by individual papers such as Blender paper \cite{Roller:20} -- summarize that our behavior labels directly address the evaluation of these issues brought up by related work and enumerate examples of such related works as justification

Human evaluation for dialogue studies \cite{Smith:22}

Recently, \newcite{Qin:21} proposed to segment consistency for task-oriented dialogue systems into three cases: dialogue history inconsistency, user query inconsistency, and knowledge base inconsistency.

Other factual consistency work: \cite{Honovich:22} \cite{Gupta:22}, \cite{Santhanam:21}

Pairwise human evaluation \cite{Li:19} \cite{Liang:20} \cite{Mohankumar:22}

Automatic methods for chatbot evaluation

Chat-oriented dialogue has been 

To address these challenges, investigating new methods of chatbot evaluation has been an active area of research in recent years (CITE). 

Dialogue likert rating scales are not grounded. The scales are a number from 1 to 5, with no clear consensus on what the characteristics are for dialogues assigned different numbers. Judgements thus become arbitrary and have high variance across raters. Overcomes the subjectivity variance by averaging across many conversations and users. But this is an expensive methodology as it requires high numbers for the average to become stabilized due to such high subjectivity (not just in conversation interpretation but also in the meaning of the likert rating itself). 

Dimensions are vague. Even a small change in the wording of the prompt for a given dimensions results in a different interpretation in what is being labelled (CITE acute-eval).

It has been claimed before (CITE ucdavis beyond likert ratings) that there is less variance in comparative judgements than in likert scale judgements. However, to our knowledge, no empirical analysis of the relative variance of each type was presented in the paper nor had been performed in earlier works. The comparative decision is more grounded than a numeric likert scale, since it is a relative judgement rather than an absolute judgement. 

For example, common methods are a 1-5 Likert rating (CITE) or the proportion of users who select one chatbot as higher quality than another (CITE).



==> tex/conclusion.tex <==
\section{Conclusion}

==> tex/excerpts/costs.tex <==
\footnote{We paid a fixed amount for the completion of each annotation task on a single dialogue. The fixed amounts were set such that annotators were paid at a \$20/hour rate as determined by pilot completion times for each annotation task. The rates were \textit{Dialogue Likert}: \$0.60, \textit{Comparative}: \$1.43, \textit{Turn Likert (one dimension)}: \$0.70,  \textit{Sociality}: \$0.44, \textit{Interpretability}: \$0.63, \textit{Empathy}: \$1.15, \textit{Personal Information}: \$0.70, \textit{Knowledge}: \$1.96, \textit{Commonsense}: \$0.92, \textit{Consistency}: \$0.87, \textit{Dialogue Flow}: \$1.87.}

==> tex/fig/behavior-labels.tex <==
\begin{table*}[ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Label}  & \textbf{Tag} & \textbf{Description} & \textbf{Subtask}  \\ \hline
Uninterpretable & \tt $\sim$Int & It is difficult to understand the intended meaning of part or all of the response. & Interpretability  \\ \hline
Antisocial & \tt $\sim$Soc & The response is insulting, hateful, or excessively vulgar. & Sociality  \\ \hline
Preference Info & \tt Pre & The response expresses the bot's preferences, wishes, or values. & Personal Information  \\ \hline
Life Info & \tt Lif & The response shares information about the bot's life or experiences. & Personal Information   \\ \hline
Empathetic & \tt Emp & The response shows an understanding and reacts appropriately to someone's emotions. & Empathy   \\ \hline
Lack of Empathy & \tt $\sim$Emp & The bot misunderstands or reacts inappropriately to someone's emotions. & Empathy   \\ \hline
Commonsense Contradiction & \tt $\sim$Com & The response misunderstands or contradicts common knowledge. & Commonsense   \\ \hline
Fact Usage & \tt Fac & The response accurately incorporates encyclopedic or expert knowledge. & Knowledge  \\ \hline
Fact Contradiction & \tt $\sim$Fac & The response hallucinates or inaccurately presents encyclopedic or expert knowledge. & Knowledge   \\ \hline
Self Contradiction & \tt $\sim$Sel & The bot contradicts something it said earlier in the dialogue. & Consistency   \\ \hline
Partner Contradiction & \tt $\sim$Par & The bot contradicts or misremembers something the user said earlier in the dialogue. & Consistency    \\ \hline
Redundant & \tt Red & The response inappropriately repeats information presented earlier in the dialogue. & Consistency    \\ \hline
Ignore & \tt Ign & The response ignores what the user just said. & Transitions    \\ \hline
Irrelevant & \tt $\sim$Rel & The response interrupts the current topic of discussion by presenting unrelated information. & Transitions \\ \hline
Follow-up & \tt Fol & The response explores, elaborates on, or asks about the ideas shared in the previous turn. & Transitions \\ \hline
Topic Switch & \tt Top & The response introduces something new to talk about. & Transitions \\
\hline
\end{tabular}
}
\caption{The 16 behavior labels within ABC-Eval. Shorthand symbols, descriptions, subtask categorization, and novelty of the labels are provided.}
\label{tab:behavior_labels}
\end{table*}

==> tex/terminal_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We hope that future work can find use in our analyses and methodology and address the challenges we quantified for MOTD chatbots.
